Social Status and Badge Design

Many websites rely on user-generated content to provide value to consumers. These websites typically incentivize participation by awarding users badges based on their contributions. While these badges typically have no explicit value, they act as symbols of social status within a community. In this paper, we consider the design of badge mechanisms for the objective of maximizing the total contributions made to a website. Users exert costly effort to make contributions and, in return, are awarded with badges. A badge is only valued to the extent that it signals social status and thus badge valuations are determined endogenously by the number of users who earn each badge. The goal of this paper is to study the design of optimal and approximately badge mechanisms under these status valuations. We characterize badge mechanisms by whether they use a coarse partitioning scheme, i.e. awarding the same badge to many users, or use a fine partitioning scheme, i.e. awarding a unique badge to most users. We find that the optimal mechanism uses both fine partitioning and coarse partitioning. When status valuations exhibit a decreasing marginal value property, we prove that coarse partitioning is a necessary feature of any approximately optimal mechanism. Conversely, when status valuations exhibit an increasing marginal value property, we prove that fine partitioning is necessary for approximate optimality.

==> approximate.tex <==
% !TEX root=badges.tex
%
%\vsdelete{In this section, we show that simple badge mechanisms can achieve a constant approximation of the output generated by the optimal mechanism, under very generic assumptions on the social status function $\stat{\cdot}:[0,1]\rightarrow \R^+$. We break our analysis based on the convexity of the status function. We show that when social status is a concave function of the proportion of players with an equal or better status class (i.e. the marginal increase in status decreases as you beat more and more players), then a single badge can achieve a $4$-approximation to the optimal mechanism. On the contrary, when status is a convex function we show examples where a logarithmic in the number of players loss is necessary for any fixed number of badges. 
%We also provide logarithmic upper bounds for several natural classes of non-concave status functions and
% give a generic upper bound that applies to any status function, stating that a number of badges that is
%logarithmic in the ratio between the highest and lowest status is sufficient.}
%
%\subsection{Decreasing Marginal Status Functions}
Concavity of the status function implies that the marginal increase from beating one extra person decreases as a player is closer to the top. For such status functions
we show that a very coarse status discrimination is sufficient to incentivize players to invest close to the optimal effort. We start by showing an approximation 
result for the very simple median badge mechanism and then show how the approximation ratio can be improved by also taking into account the monopoly quantile
of the specific distribution at hand.

\begin{theorem}[Median Absolute Badge Mechanism]\label{thm:concave} If the social status function $\stat{\cdot}$ is concave, then a single badge, with quantile threshold equal to $1/2$, can achieve a $4$-approximation to the optimal revenue. 
\end{theorem}
\begin{proof}
Let $OPT$ denote the revenue  of the optimal mechanism and $APX$ the revenue of the single badge mechanism. 
A single badge mechanism at quantile $\tq{}$ achieves revenue of 
\begin{equation}
APX = n\cdot R(\tq{}) \cdot \statn{n}{\tq{}},
\end{equation}
while the optimal mechanism gets revenue:
\begin{equation}\label{eqn:opt-reminder}
OPT = n\cdot  \int_0^{\tqstar} R'(\quant)\cdot\statn{n}{\quant}d\quant \leq n\cdot \statn{n}{0} \int_0^{\tqstar} R'(\quant)d\quant  = n\cdot \statn{n}{0}\cdot R(\tqstar)
\end{equation}
By setting $\tq{}=1/2$, and by the concavity of the revenue function we have:
\begin{equation}
R(1/2) \geq \int_0^{1} R(\quant)d\quant
\end{equation}
Additionally, since $R(\cdot)$ is concave and $R(0)=R(1)=0$, it is easy to see that $\int_0^1 R(\quant)d\quant \geq \frac{1}{2}\cdot R(\tqstar)$\footnote{This is the same argument
employed for proving the statement that the revenue of the optimal single item auction with a single bidder yields lower revenue than the second price auction with two i.i.d bidders. See Figure 5.1 in \cite{Hartline2012}}. Last, since $\statn{n}{\cdot}$ is concave decreasing and $\statn{n}{1}=0$, we get $\statn{n}{1/2}\geq \frac{1}{2}\statn{n}{0}$. Combining all the above facts, yields the theorem.
\end{proof}

\begin{example}[Tight lower bound for median badge mechanism] Consider the case of a linear status function $\stat{t}=1-t$ and a distribution of abilities with density function $F(\val)=\frac{H+1}{H}\frac{\val}{\val+1}$ and support
$[0,H]$. The value function of this distribution is $\val(\quant)=\frac{1-\quant}{\frac{1}{H}+\quant}$ and the revenue function is $R(\quant)=\frac{\quant}{\frac{1}{H}+\quant}\cdot (1-\quant)$. As $H\rightarrow \infty$ (abilities are very dispersed but most of the mass is at the lower end) the revenue curve converges to $R(\quant)\rightarrow (1-\quant)$ and the optimal total contribution converges to $n$. On the other hand the total contribution of the median badge converges to $\frac{n}{4}$.
\end{example}

\begin{theorem}\label{thm:concave} If the social status function $\stat{\cdot}$ is concave, then a single badge, with quantile threshold equal to $\min\{\tqstar,1/2\}$, can achieve a $3$-approximation to the optimal revenue. (proof in Appendix)
\end{theorem}


%\begin{theorem}\label{thm:concave} If the social status function $\stat{\cdot}$ is concave, then a single badge, with quantile threshold equal
%to half the monopoly quantile, can achieve a $4$-approximation to the optimal revenue. 
%\end{theorem}
%\begin{proof}
%%Summarizing the analysis in the previous two sections we know that the optimal mechanism achieves revenue of:
%%\begin{equation}
%%OPT= n\left(R(\kappa^*)\cdot \hat{x}(\kappa^*)-\int_{0}^{\kappa^*}R(q)\hat{x}'(q)dq\right)
%%\end{equation}
%%where $\hat{x}(q) =  \sum_{\nu=0}^{n-1}f\left(\frac{\nu+1}{n}\right)\beta_{\nu,n-1}(q)$.
%Let $OPT$ denote the revenue  of the optimal mechanism and $APX$ the revenue of the single badge mechanism. 
%A single badge mechanism at quantile $\tq{}$ achieves revenue of 
%\begin{equation}
%APX = n\cdot R(\tq{}) \cdot \xq{\tq{}}
%\end{equation}
%We will show that if we set $\tq{}=\frac{\tqstar}{2}$ then $4\cdot APX\geq OPT$.
%
%First we point out that if the social status function is concave, then $\xq{\quant}$ is also a concave function. This follows 
%from known facts about binomial distributions and derivatives of Bernstein polynomials. Thus $\xq{\quant}$
%is a decreasing concave function of $\quant$. From this fact it follows that:
%\begin{equation}
%\xq{\frac{\tqstar}{2}}\geq \frac{\xq{0}+\xq{\tqstar}}{2} \geq \frac{\xq{0}}{2}
%\end{equation}
%
%Additionally, by regularity of the distribution we know that $R(q)$ is a concave function and additionally, for any $\quant\leq \tqstar$, $R(\quant)$ is increasing (since, $\tqstar$ is defined as the point where $R'(\tqstar)=0$). Additionally, $R(0)=0$.
%From this it follows that:
%\begin{equation}
%R\left(\frac{\tqstar}{2}\right)\geq \frac{R(\tqstar)}{2}
%\end{equation}
%Combining the two we get that the revenue of the single badge mechanism is at least:
%\begin{equation}
%APX\geq n\cdot\frac{R(\tqstar)\cdot \xq{0}}{4}
%\end{equation}
%
%By the fact that $R(\quant)$ is increasing in the region $[0,\tqstar]$ we have that $R(\quant)\leq R(\tqstar)$. Since $\xq{\quant}$
%is decreasing in $\quant$ (i.e. $\xqpr{\quant}\leq 0$) we have that: $R(\quant)\xqpr{\quant}\geq R(\tqstar)\xqpr{\quant}$. Thus, we can also upper bound the revenue of the optimal mechanism:
%\begin{equation}
%OPT \leq n\left(R(\tqstar)\cdot \xq{\tqstar}-R(\tqstar)\int_{0}^{\tqstar}\xqpr{\quant}dq\right) = n\cdot R(\tqstar)\cdot \xq{0}
%\end{equation}
%The theorem then follows.
%\end{proof}



%\vsdelete{Another status function that we can apply the above theorem is the following:
%\begin{equation}
%\stat{t} = \frac{1}{n\cdot t}+\frac{1}{n\cdot t+1}+\ldots+\frac{1}{n}=H_{n}-H_{n\cdot t-1}
%\end{equation}
%The intuition behind the above social status function is the following: each social rank can be thought of as unlocking 
%priviledges or features of a web service, or in more general contest settings as unlocking some resource. Assume that each resource can  be thought as a unit of value that is shared among the players to  whom the resource is unlocked. This exact intuition is portrayed in the above function.
%Observe that this function satisfies the property that $\frac{\stat{1/n}}{\stat{1}} = n\cdot H_n$. Thus applying Theorem \ref{thm:general-function} we get that $\log(n)+\log\log(n)=O(\log(n))$ badges are sufficient to get a constant approximation 
%to the optimal revenue.}

%\vscomment{The following section is just some notes. To be taken out.}
%\subsection{Monotone Hazard Rate Ability Distributions}
%\begin{equation}
%\E_v[b(v)]=\E[\phi(v)\tilde{x}(v)]\geq \E[v\cdot \tilde{x}(v)]-\E[\eta\cdot \tilde{x}(v)]
%\end{equation}
%Additionally, if $a_1=\eta$ (see Figure \ref{fig:relation})
%\begin{equation}
%\E_v[b(v)] \geq \E[\eta \cdot \tilde{x}(v)]
%\end{equation}
%Thus:
%\begin{equation}
%\E_v[b(v)]\geq \frac{1}{2}\E[v\cdot \tilde{x}(v)]
%\end{equation}
%Thus as long as the badge mechanism approximates well the optimal welfare optimal mechanism among people above the monopoly reserve, then we are fine. 
%
%In the case of asymmetric ability distribution we have:
%\begin{equation}
%\E_{v_i}[b_i(v_i)]=\E[\phi_i(v_i)\tilde{x}_i(v_i)]\geq \E[v_i\cdot \tilde{x}_i(v_i)]-\E[\eta_i\cdot \tilde{x}_i(v_i)]
%\end{equation}
%Now by setting a single reserve in the 

%\subsection{Convexity of Approximate Badge Thresholds}
%
%In this section we show that the approximate thresholds used in our approximation theorem induce badge thresholds that have a convex form: i.e. 
%the threshold difference between consecutive intervals is increasing. This property is observed heavily in practice, since most badge thresholds in 
%question and answer forums have such convex behavior. Hence, this gives a theoretical foundation behind such badges.
%
%\begin{theorem}
%If quantile thresholds are of the form $\kappa_j = \frac{\kappa_1}{\alpha^{j-1}}$ for some $\alpha>1$, then $\theta_j-\theta_{j-1}$ is increasing in $j$.
%\end{theorem}
%\begin{proof}
%By Equation \eqref{eqn:value-to-effort} that relates value thresholds to badge thresholds, we have that if badge thresholds $\theta=(\theta_1,\ldots,\theta_m)$ implement quantile thresholds $\kappa=(\kappa_1,\ldots,\kappa_m)$ then it must hold that:
%\begin{equation*}
%v(\kappa_j)\left(\hat{x}(\kappa_j)-\hat{x}(\kappa_{j-1})\right) = \theta_j - \theta_{j-1}
%\end{equation*}
%Since value is decreasing in quantile, and $\kappa_j\geq \kappa_{j+1}$, to show that $\theta_j-\theta_{j-1}$ is increasing in $j$ it suffices
%to show that $\hat{x}(\kappa_j)-\hat{x}(\kappa_{j-1})$ is increasing in $j$. Equivalently, for all $j\in [2,m-1]$
%\begin{equation*}
%\hat{x}(\kappa_j)-\hat{x}(\kappa_{j-1})\leq \hat{x}(\kappa_{j+1})-\hat{x}(\kappa_j) \Leftrightarrow 2\hat{x}(\kappa_j)\leq \hat{x}(\kappa_{j+1})+\hat{x}(\kappa_{j-1})
%\end{equation*}
%
%We first observe that:
%$$\kappa_{j+1}+\kappa_{j-1} = \frac{\kappa_1}{\alpha^{j}}+\frac{\kappa_1}{\alpha^{j-2}} = \frac{\kappa_1}{\alpha^{j-1}}\left(\frac{1}{\alpha}+\alpha\right)\geq 2\cdot \kappa_j $$
%Since interim allocation is non-increasing in quantile we have:
%\begin{equation}
%\hat{x}(\kappa_j) \geq \hat{x}
%\end{equation}
%\end{proof}
























==> argument.tex <==
% !TEX root=badges.tex
Implicit in our utility model so far is that players treat people in the same class as them, as if they were losing to them, since
they affected a players utility in an equal manner as players strictly above them. How do our results change qualitatively if 
instead players treated ties differently. We examine two alternative models, in the first players treat ties as if they were beating them and in the second one tied players are treated as above or below with probability equal.

The second alternative is rather meaningful in the context of Q\&A forum where status can be interpreted as argumentative power. We can think of status utility as the probability that a player wins in an argument against a random other user from the system. In most such systems, the credibility derived from having a badge plays a quintessential role in deciding who wins the argument (e.g. voted best answer, presented at the top of the page). Our status utility assumes that a player with a strictly higher badge status will win an argument. Additionally, the tie-breaking rule in the status utility function corresponds to the probability that a player wins against an opponent with equal status. Our model so far assumed that in such battles, even if
there is a winner, his victory is Pyrrhic, and no player ends up getting any utility. The alternative model corresponds to 
each player winning with equal probability.

Given the latter interpretation we explore the qualitative change in our results mainly for the case of linear status. Thus
if we denote with $t_g$ the proportion of other players that are strictly higher than player $i$ and with $t_e$ the proportion
of other players that are tied with player $i$, then the status utilities that we will analyze are:
\begin{align}
S(t_e, t_g)=1-t_g\\
S(t_e,t_g)=1-t_g-\frac{t_e}{2}
\end{align}
Our initial model corresponds to the case: $S(t_e,t_g)=1-t_g-t_e$. Other than that, the utility of a player is the same as defined in Section \ref{sec:model}, i.e. if $t_e^i(b), t_g^i(b)$ is the corresponding proportions for player $i$ under a bid profile $b$, then:
\begin{equation}
u_i(b;v_i) = S(t_e^i(b),t_g^i(b))-\frac{b_i}{v_i}
\end{equation}
\vsedit{In this alternative models, we avoid setting the status of a player that receives no badge to $0$, since under
the interpretation we want to capture, even players that are at the last social status class, still are winning with positive probability when facing other players with no badge.}

\subsection{Random Winner}

In this setting we first observe that the optimal mechanism is slightly altered. Specifically, it is no longer the case that players below the monopoly reserve are simply assigned rank $0$. Under the initial model, to maximize virtual welfare, if a player had negative virtual value, then we should simply assign him as low status as possible, and that is feasible by putting him at the lowest rank and thereby assigning him the status equal to the status of the lowest ability player. 

However, when players that tie win each with probability half, then grouping together negative virtual value players is no longer optimal. Specifically, we would always increase utility by separating even low ability players. The proof is clear when viewed under the argument battle interpretation of status. Observe that the virtual welfare collected under some rank assignment is the expected virtual value of the winners from the random argument matchings. In the initial model we had that in the case of ties, no player is a winner. Thus the optimal would have been to group together all negative virtual value players in the bottom, so that no such player is ever a winner of a battle and hence we don't collect his negative virtual value. However, in the alternative tie-breaking rule, these players are win with equal probability. Hence, we would rather have the higher virtual value player win even if his virtual value is negative. This leads to the following Lemma.

\begin{lemma} When social status is $S(t_e,t_g)=1-t_g-\frac{t_e}{2}$, the optimal mechanism assigns a distinct rank to all players in decreasing order of value (or equivalently bid).
\end{lemma}

Thus under the optimal mechanism no two players tie with each other. The interim allocation of the optimal mechanism, in quantile space is then simply:
\begin{equation}
\xq{\quant[i]}= 1- \quant[i]
\end{equation}
while the revenue of the optimal mechanism is simply:
\begin{equation}
OPT = - n\int_0^1 R(\quant) \xqpr{\quant}d\quant = n \int_0^1 R(\quant)d\quant
\end{equation}

Now we consider how the equilibrium and revenue characterization of a badge mechanism is altered. First observe that 
the equilibrium is still going to be a step function and thereby there will still be a one-to-one correspondence between
badge thresholds and quantile thresholds. The relation between badge thresholds and quantile thresholds will 
be given by an equivalent relation to Equation \eqref{eqn:value-to-effort},
\begin{equation}
\theta_t-\theta_{t-1}=\val(\tq{t})(\hat{x}^{\theta}(\tq{t})-\hat{x}^\theta(\tq{t-1}))
\end{equation} 
However, now $\hat{x}^{\theta}(\tq{t})$ will not correspond to the interim allocation of a player with quantile $\kappa_t$ under the optimal mechanism.
Instead $\hat{x}^{\theta}(\tq{t})$ will correspond to the interim allocation of a player with badge $t$. Under the linear status model, this is simply 
\begin{equation}
\hat{x}^{\theta}(\tq{t})=1-\tq{t+1}-\frac{\tq{t}-\tq{t+1}}{2}=1-\frac{\tq{t}+\tq{t+1}}{2}
\end{equation}
with $\hat{x}^\theta(1)=\frac{\tq{1}}{2}$. Thus the relation between badge and quantile thresholds becomes:
\begin{equation}
\theta_t-\theta_{t-1}=\val(\tq{t})\left(\frac{\tq{t-1}+\tq{t}}{2}-\frac{\tq{t}+\tq{t+1}}{2}\right)=\val(\tq{t})\left(\frac{\tq{t-1}-\tq{t+1}}{2}\right)
\end{equation}

For the case of many badges, we can no longer solve for the quantile thresholds, given a badge threshold mechanism (the converse is trivial), using a recursive approach as in Section \ref{sec:equilibrium}. However, the latter is easy for the case of a single badge where the relation is simply:
\begin{equation}
\theta_1 = \frac{\val(\tq{1})}{2}
\end{equation}
Additionally, the revenue of a single badge mechanism with quantile thresholds $\tq{t}$ is simply: 
\begin{equation}
\E\left[\sum_i b_i(v_i)\right]=n\cdot \tq{1}\cdot \tb{1}=n\cdot \frac{R(\tq{1})}{2}
\end{equation}
By picking the monopoly quantile threshold, which is the quantile that maximizes the revenue function $R(\cdot)$, it is easy to see that the latter revenue is at least half of the optimal revenue.
\begin{theorem}
When social status is $S(t_e,t_g)=1-t_g-\frac{t_e}{2}$, a single badge mechanism with the monopoly quantile threshold $\tqstar$ achieves at least half of the revenue of the optimal mechanism.
\end{theorem}

\subsection{Everyone is a Winner}

\begin{theorem} When $S(t_e, t_g)=1-t_g$, the optimal mechanism is a single badge mechanism, with badge threshold $\theta=R(\tqstar)$ and quantile threshold $\tqstar$.
\end{theorem}
\begin{proof}
Based on the random matching and argument interpretation of the status, the best possible virtual welfare that a mechanism can achieve is to always collect the virtual values of both players when their virtual values are positive and never collect them
when they are negative. It is easy to see that the mechanism that assigns rank $1$ to all players with ability above the monopoly
quantile and a rank of $0$ to all players with ability below, achieves exactly this optimal virtual welfare. Such an allocation function
can be achieved by a single badge mechanism with badge threshold $\theta=\val(\tqstar)\tqstar$. The latter stems from the fact that for a player with quantile $\tqstar$ to be indifferent, it must be that his net gain from moving from badge $0$ to badge $1$, which is $\val(\tqstar)(1-(1-\tqstar))$, is equal to his net increase in cost, which is $\theta$.
\end{proof}











==> asymmetric.tex <==
% !TEX root=badges.tex

In this section we consider the case of asymmetric bidder distributions. We characterize the equilibrium of the game
when the number of players drawn from each distribution goes to infinity and we show that in the limit the 
equilibrium induced by a badge mechanism is completely symmetric. In other words, the equilibrium is characterized
by a set of ability thresholds $\tv{1},\ldots,\tv{m}$ that correspond to each badge threshold and such that players
with ability $v\in [\tv{t},\tv{t+1}]$ bid threshold $\tb{t}$ independent of the distribution that they belong too.

The large market limit of the asymmetric market can be thought as follows: there are $k$ different populations. The ability of each bidder 
in population $j$ is drawn from a distribution with CDF $\acdf{j}{}$
and support $[0,\bar{\val}_j]$.  We take the limit of the large market as follows: we assume that in the limit each population $j$
will constitute a $p_j$ fraction of the market. Thus we consider a limit process where as the size $n$ of the total population
goes to infinity, then the empirical frequency of each population $j$ goes to $p_j$, i.e. $\frac{n_j}{n}\rightarrow p_j$.

Consider a badge mechanism defined by a set of thresholds $\tb{1},\ldots,\tb{m}$. We will analyze the equilibrium behavior induced
 by the mechanism and will focus on the equilibrium where the bid function is symmetric among players in the same population. Thus
we denote with $b_j(\cdot)$ this equilibrium bid function. It is easy to observe that $b_j(\cdot)$ will still be a step function
as in the symmetric case and hence will be characterized by a set of ability thresholds $\tv{1}^j,\ldots,\tv{m}^j$ such that players
with ability $v\in [\tv{t}^j,\tv{t+1}^j]$ will bid $\tb{t}$. However, in the asymmetric setting the ability thresholds $\tv{t}^j$ are
potentially different for different populations. We will show that although this may be the case for any finite population game, in the
limit of an infinite population, the ability thresholds are the same for all populations, and hence the equilibrium ends up being a symmetric one.

We first examine the interim utility of a bidder $i$ in population $j$. If he has an ability $v\in [\tv{t}^j,\tv{t+1}^j]$ then he gets badge $t$
and his social status is a function of the proportion of people that have badge at least as high as $t$. This accounts to the summation over
all populations of  the players from each population $j'$ that have value at least $\tv{t}^{j'}$. More formally, 
if we are at a finite vector of populations, $n_1,\ldots,n_k$, from the perspective of any player $i$ in population $j$, the expected proportion of people
that have badge at least as high as $t$ is:
\begin{equation}
\E\left[\frac{|i':b_{i'}(\tv{i'})\geq \tb{t}|}{n}~\bigg|~\val[i]\in [\tv{t}^j,\tv{t+1}^j]\right]=\frac{1}{n}+\frac{n_j-1}{n} \left(1-\acdf{j}{\tv{t}^j}\right)+\sum_{j'\neq j}\frac{n_{j'}}{n}\left(1-\acdf{j'}{\tv{t}^{j'}}\right)
\end{equation}
In the large market limit, the above fraction converges to the following expression that is the same from the perspective of any player:
\begin{equation}
\E\left[\frac{|i':b_{i'}(\tv{i'})\geq \tb{t}|}{n}~\bigg|~\val[i]\in [\tv{t}^j,\tv{t+1}^j]\right]\rightarrow \sum_{j=1}^{k}p_j \cdot \left(1-\acdf{j}{\tv{t}^j}\right)
= 1-\sum_{j=1}^{k}p_j\cdot\acdf{j}{\tv{t}^j}
\end{equation}
Additionally, the actual proportion of players converges to the above expectation, and therefore in the limit we can assume that the proportion of players
that have badge at least $t$ is the latter expectation. Therefore, the interim allocation of any player in population $j$ with value $\val\in[\tv{t}^j,\tv{t+1}^{j}]$,
ends up:
\begin{equation}
\tilde{x}^j(v) =\stat{1-\sum_{j=1}^{k}p_j\cdot \acdf{j}{\tv{t}^j}}=c_t(\tv{t}^1,\ldots,\tv{t}^m)
\end{equation}
which is some function that is independent of the population $j$, but only a function of the badge $t$.

By the equilibrium conditions for each population we have that the population specific ability thresholds have to satisfy similar conditions as
in the symmetric case, i.e.
\begin{align*}
\tv{1}^j \tilde{x}^j(\tv{1}^j)=~&\tb{1}\\
\tv{t}^j \cdot (\tilde{x}^j(\tv{t}^j)-\tilde{x}^j(\tv{t-1}^j))=~&\tb{t}-\tb{t-1} & \forall t\in[2,m]
\end{align*}
Since $\tilde{x}^j(\tv{t}^j)=c_t(\tv{t}^1,\ldots,\tv{t}^m)$ we get:
\begin{align*}
\tv{1}^j =~& \frac{\tb{1}}{c_1(\tv{1}^1,\ldots,\tv{1}^m)}\\
\tv{t}^j = ~& \frac{\tb{t}-\tb{t-1}}{c_t(\tv{t}^1,\ldots,\tv{t}^m)-c_{t-1}(\tv{t-1}^1,\ldots,\tv{t-1}^m)} & \forall t\in [2,m]
\end{align*}
which then implies that the ability thresholds are identical for all populations, i.e. $\tv{t}^j=a_j$, since the right hand sides on the above set of equations are independent of the population $j$. We will then denote with:
\begin{equation}
c_t(\tv{t})=\stat{1-\sum_{j=1}^{k}p_j\cdot \acdf{j}{\tv{t}}}
\end{equation}
and therefore, the ability thresholds are characterized by the set of equations:
\begin{align}\label{eqn:asymmetric-thresholds}
\tv{1}\cdot c_1(\tv{1})=~& \tb{1}\\
\tv{t}\cdot (c_t(\tv{t})-c_{t-1}(a_{t-1}))=~&\tb{t}-\tb{t-1} & \forall t\in [2,m]
\end{align}

To simplify the analysis we denote with $\cdf[a]=\sum_{j=1}^{k}p_j\cdot \acdf{j}{a}$, to be the aggregate distribution
of the total population. Similarly we denote with $\quant(a)=1-\cdf[a]$ to be the quantile function of the aggregate distribution
and with $\val(\quant)$ the inverse quantile. Last we denote with $R(\quant)=\quant\cdot \val(\quant)$ the revenue function of the aggregate
distribution. 

By the above analysis we get that a set of uniform ability thresholds $\tv{1},\ldots,\tv{m}$ corresponds to a set of quantile thresholds $\tq{1},\ldots,\tq{m}$ in the quantile space of the aggregate distribution. The quantile thresholds are related with the badge thresholds via:
\begin{align}\label{eqn:asymmetric-thresholds}
\val(\tq{1})\cdot \stat{\tq{1}}=~& \tb{1}\\
\val(\tq{t})\cdot (\stat{\tq{t}}-\stat{\tq{t-1}})=~&\tb{t}-\tb{t-1} & \forall t\in [2,m]
\end{align}
%
%\begin{example}
%To illustrate the relation between badge thresholds and ability thresholds we give a concrete example. Consider the instance, where
%each population $j$ is distributed uniformly, $U[0,\beta_j]$, but with population specific supports and assuming $\bet\tv{1}\leq \ldots\leq \beta_k$. Additionally, consider the  linear social status function $f(t)=1-t$ described in the previous sections and that the badge mechanism has only one badge. In this setting the interim allocation of a player that gets badge $1$ is: 
%\begin{equation}
%c_1(\tv{1})= \sum_{j=1}^k p_j \cdot F_j(\tv{1})=\sum_{j=1}^k p_j \cdot \frac{\tv{1}}{\beta_j}=\tv{1} \sum_{j=1}^k \frac{p_j}{\beta_j}
%\end{equation}
%as long as $\tv{1}\leq \bet\tv{1}$. More generally, if $\tv{1}\in [\beta_r,\beta_{r+1}]$ then we get:
%\begin{equation}
%c_1(\tv{1})= \tv{1}\left(\sum_{j<r+1}p_j + \sum_{j\geq r+1}\frac{p_j}{\beta_j}\right)
%\end{equation}
%By the set of Equations \eqref{eqn:asymmetric-thresholds} we get that:
%\begin{align*}
%\tv{1}=~&\sqrt{\frac{\tb{1}}{\left(\sum_{j<r+1}p_j + \sum_{j\geq r+1}\frac{p_j}{\beta_j}\right)}}
%\end{align*}
%Dependent on $\tb{1}$ we can find $r$ such that the solution to the above equation is in the region $[\beta_r,\beta_{r+1}]$.
%\end{example}


\subsection{Designing Badge Mechanisms in Large Asymmetric Markets}
The above analysis tells us that in the limit of a large asymmetric market, designing a badge mechanism, essentially, is equivalent to finding a set of $m$ quantile thresholds $\tq{1},\ldots,\tq{m}$, in the quantile space of the aggregate distribution, that maximize revenue
%, assuming that every player, irrespective of distribution, will bid get
%badget $t$ if his ability is in the region $[\tv{t},\tv{t+1}]$.
%In some sense, a badge mechanism allows us to implement almost any symmetric direct revelation mechanism.
%
%The question of approximate optimality then boils down to the approximate optimality of the above symmetric ability threshold mechanisms. Observe that a symmetric vector of ability thresholds doesn't imply a symmetric vector of quantile thresholds.
%
%For instance, in the case of uniform distributions with different support upper bounds, a uniform ability threshold of $a$ corresponds to a set of quantile thresholds $k^j=\beta_j-a$.

Since we are interested in the infinite player limit, to avoid coping with infinite revenue, we will equivalently, consider 
the problem of maximizing the per player revenue. Following similar analysis as in Section \ref{sec:equilibrium} we get that the 
revenue of a badge mechanism defined by a set of quantile thresholds $\tq{1},\ldots, \tq{m}$ is:
\begin{align}
\E_{\val}\left[\frac{1}{n}\sum_i b_i(\val[i])\right] 
%=~& \sum_{j=1}^{k} p_j \sum_{t=1}^{m} R_j(\tq{t}^j)\cdot (c_t(\tv{t})-c_{t-1}(a_{t-1}))\\
%=~&\sum_{t=1}^{m} (c_t(\tv{t})-c_{t-1}(a_{t-1}))\sum_{j=1}^{k} p_j R_j(\tq{t}^j)\\
=~&\sum_{t=1}^{m} \left(\stat{\tq{t}}-\stat{\tq{t-1}}\right)\cdot R(\tq{t})\nonumber\\
=~& R(\tq{m})\cdot \stat{\tq{m}}+ \sum_{t=1}^{m-1} (R(\tq{t})-R(\tq{t+1}))\cdot \stat{\tq{t}}\label{eqn:discrete-revenue-equiv}
\end{align}
%If we denote with $q(a)=\sum_{j=1}^{k} p_j \kappa_j(a)$ to be the expected proportion of players above a given ability $a$, then the above simplifies to:
%\begin{align*}
%\E_{v}\left[\frac{1}{n}\sum_i b_i(v_i)\right] =~& \sum_{t=1}^m \left(f(q(\tv{t}))-f(q(a_{t-1}))\right)\cdot q(\tv{t}) \cdot \tv{t}
%\end{align*}
For a single badge with a quantile thresholds of $\tq{}$, the above is simply: $\stat{\tq{}}\cdot R(\tq{})$. 

On the other hand the optimal mechanism, is rather complicated, since it doesn't treat the players from the different populations in a symmetric way. Hence, a player might be winning, despite having lower value than some other player in another population. 
More specifically, the optimal mechanism orders players in decreasing order of virtual value, which is no longer the same as 
decreasing order of value. 

Comparing a badge mechanism with such a discriminatory auction is rather unfavorable. Instead we will analyze the revenue of 
a single badge mechanism with that of a continuum of badges, which essentially, can simulate any monotone, symmetric mechanism. We show that the $4$-approximation that we showed in the symmetric setting carries over to this setting too.

\begin{theorem} In the limit of infinite players, a single badge mechanism is a $4$-approximation to any badge mechanism
with an arbitrary number of badges, when the status function is concave.
\end{theorem}
\begin{proof}
Consider an optimal badge mechanism with $m$ badges and denote with $OPT^m$ its average per player revenue. From Equation \eqref{eqn:discrete-revenue-equiv} we see that the optimal badge mechanism for any number of badges $m$,  never has a quantile threshold $\tq{1}\geq \kappa^*$, where $\kappa^*$ is the monopoly quantile of the aggregate distribution. The reasoning is that after $\kappa^*$ the revenue function is decreasing. It is trivial to see that the quantity in 
 Equation \eqref{eqn:discrete-revenue-equiv} can always be strictly improved if instead we set all quantile thresholds above $\kappa^*$ to be exactly equal to $\kappa^*$. Thus the coefficients of each $f(t)$ are positive numbers. Subsequently, 
since $f(q)$ is decreasing in $q$, we get:
\begin{equation}
OPT^m \leq f(\tq{m})\cdot R(\tq{1})\leq f(0)\cdot R(\kappa^*)
\end{equation}

On the other hand, if we use a single badge mechanism with $\kappa=\kappa^*/2$ then following similar analysis as in 
the proof of Theorem \ref{thm:concave} we get that it achieves revenue at least: $\frac{f(0)\cdot R(\kappa^*)}{4}$, which completes the proof.
\end{proof}

%Hence, for any value $v$ of a player from population $j$, his interim allocation is $f(t)$ where
%$t$ where $t$ is the proportion of people with higher virtual value than player $i$. This interim allocation still inherits the convexity properties of the status function $f(\cdot)$. Thus $\hat{x}_j(q_j)$ will still be a decreasing concave function if $f(\cdot)$ is a concave function. \vscomment{The latter needs to be checked slightly more formally.}
%
%The expected per player revenue of the optimal mechanism will then be:
%\begin{align*}
%\frac{1}{n} OPT =~& \sum_{j=1}^{k}p_j\cdot \left(R_j(\kappa_j^*)\hat{x}_j(\kappa_j^*)-\int_{0}^{\kappa_j^*}R_j(q)\hat{x}_j'(q)dq\right)
%\end{align*}
%By regularity of each distribution $F_j$ and using similar reasoning as in Theorem \ref{thm:concave} the latter is at most:
%\begin{align*}
%\frac{1}{n} OPT \leq~& \sum_{j=1}^{k}p_j\cdot R_j(\kappa_j^*)\cdot \hat{x}_j(0)
%\end{align*}
%
%For simplicity assume that all distributions have the same support. Thus a quantile of $0$ corresponds to the same ability $\bar{v}$ for every distribution. Additionally, $\hat{x}_j(0)=f(0)$ for every distribution. Thus:
%\begin{align*}
%\frac{1}{n} OPT\leq~& f(0) \sum_{j=1}^{k}p_j\cdot R_j(\kappa_j^*) =  f(0) \sum_{j=1}^{k}p_j\cdot \kappa_j^*\cdot a_j^* 
%\end{align*}
%Let $Q=\sum_{j=1}^{k}p_j\cdot \kappa_j^*$ be the expected proportion of people that are being given a non-zero rank.
%

%\subsection{Asymmetric Badges} So far we analyzed the guarantees achievable by a badge mechanism in an asymmetric environment. Deriving intuition from optimal mechanisms, we know that in an asymmetric environment the optimal
%mechanism must treat players from different distributions asymmetrically. Thus in an asymmetric environment 
%a badge mechanism can potentially achieve higher revenue if it treats different populations differently. 
%
%Thus we analyze the revenue of badge mechanisms where different populations face different badge thresholds. Such a badge
%mechanism is defined by a set of thresholds $\tb{1}^j,\ldots,\tb{m}^j$ for each population $j$. The equilibrium conditions, thus become:
%\begin{align*}
%\tv{1}^j \tilde{x}^j(\tv{1}^j)=~&\tb{1}^j\\
%\tv{t}^j \cdot (\tilde{x}^j(\tv{t}^j)-\tilde{x}^j(a_{t-1}^j))=~&\tb{t}^j-\theta_{t-1}^j & \forall t\in[2,m]
%\end{align*}
%Thus observe that for any set of asymmetric ability thresholds $\tv{1}^j,\ldots,\tv{m}^j$ there exist a set of asymmetric badge
%thresholds that implement them at equilibrium. 

















==> comparative.tex <==
% !TEX root=badges.tex

\begin{theorem} Consider two status functions $S_1(\cdot)$ and $S_2(\cdot)$, such that $S_1(\cdot)$ is convex,
$S_2(\cdot)$ is concave, $S_1(1)=S_2(1)=0$ and the expected social welfare of the optimal mechanism is identical:
\begin{equation}
\int_0^{\tqstar} \val(\quant) \hat{x}_1(\quant)d\quant=\int_0^{\tqstar} \val(\quant) \hat{x}_2(\quant)d\quant
\end{equation}
where:
\begin{equation}
\hat{x}_r(\quant)=\sum_{\nu=0}^{n-1}S_r\left(\frac{\nu+1}{n}\right)\beta_{n-1, \nu}(\quant)
\end{equation}
If the ability distribution satisfies the Monotone Hazard Rate condition, then the optimal revenue under $S_1(\cdot)$
is higher than the revenue under $S_2(\cdot)$.
\end{theorem}
\begin{proof}
Observe that $\hat{x}_1(\cdot)$ is convex, $\hat{x}_2(\cdot)$ is concave, $\hat{x}_1(1)=\hat{x}_2(1)=0$. Thus there are
only two cases: 1) either $\hat{x}_1(\cdot)$ lies strictly above $\hat{x}_2(\cdot)$ in the region $[0,1]$ or 2) $\hat{x}_1(\cdot)$
lies below $\hat{x}_2(\cdot)$ in a region $[t,1]$ and lies above in the region $[0,t]$.

By the equal welfare property:
\begin{equation}
\int_0^{\tqstar} \val(\quant) \cdot \left(\hat{x}_1(\quant)-\hat{x}_2(\quant)\right)d\quant=0
\end{equation}
Since $\val(\quant)$ is a non-negative function, it must be that only the second case is valid. Thus if we denote with
$g(q)=\hat{x}_1(\quant)-\hat{x}_2(\quant)$, then $g(q)$ is positive in the region $[0,t]$ and negative in $[t,1]$ and $t\in[0,\tqstar]$.

Since $\val(\quant)$ is decreasing, it is then implied that:
\begin{equation}\label{eqn:diff-negative}
\int_0^{\tqstar} g(\quant)d\quant = \int_0^{\tqstar}  \hat{x}_1(\quant)-\hat{x}_2(\quant)d\quant<0
\end{equation}
The difference in optimal per-player revenue under the two functions is:
\begin{align*}
\E[p_1(\quant)-p_2(\quant)]=~&\int_0^{\tqstar} R'(\quant) g(\quant)d\quant\\
=~&\int_0^{\tqstar} \val(\quant) \cdot g(\quant) d\quant+\int_0^{\tqstar} q \cdot \val'(\quant) \cdot g(\quant)d\quant\\
=~&\int_0^{\tqstar} q\cdot \val'(\quant) \cdot g(\quant)d\quant
\end{align*}
Since $\val(\quant)$ is decreasing, $-\quant\val'(\quant)\geq 0$. If $-\quant\val'(\quant)$ is increasing, then following
Equation \eqref{eqn:diff-negative} and the properties of $g(\quant)$ we have:
\begin{align*}
\int_0^{\tqstar} (-q\cdot \val'(\quant)) \cdot g(\quant) d\quant<0
\end{align*}
since the positive parts of $g(q)$ are amplified less than the negative parts. Thus we get that:
\begin{align*}
\E[p_1(\quant)-p_2(\quant)]=\int_0^{\tqstar} q\cdot \val'(\quant) \cdot g(\quant)d\quant>0
\end{align*}
\end{proof}







==> concave.tex <==
% !TEX root=badges.tex



==> convex-many.tex.old.tex <==
% !TEX root=badges.tex 
In this section we analyze the contributions generated by absolute badge mechanisms for settings where status valuations are convex. Unlike the linear and concave cases, we find that a single badge is insufficient for a good approximation and that any mechanism with a constant number of badges fails to achieve a constant approximation ratio. 


 
The prototypical such status function that we will analyze is the case where the status of a player is inversely proportional to 
the proportion of players (including the player himself) with a weakly better status class:
\begin{equation}
\stat{t} =\frac{n}{(n-1)t+1}-1
\end{equation}
We start by portraying that for such a function a logarithmic in the number of players loss is necessary if the number
of badges is constant.

\begin{example}{(Logarithmic Loss)} 
%We give an example portraying that for the case of $f(t)=1/t$ the optimal mechanism with $m$ badges, cannot achieve more than a $O(\log(n)/m)$ fraction of the optimal revenue. Therefore, showing that $O(\log(n))$ badges are required to achieve a constant factor of the optimal mechanism.
Consider the case where ability is distributed uniformly in $[0,1]$. The revenue function is then $R(\quant)=\quant(1-\quant)$, with derivative $R'(\quant)=1-2\cdot \quant$ and the monopoly quantile is $1/2$. Additionally, the interim allocation of a player with quantile $\quant$ under the optimal mechanism ends up being after simplifications $\xq{\quant}=\frac{1-(1-\quant)^n}{\quant}-1$. Thereby the optimal revenue is:
\begin{align*}
\frac{OPT}{n} =~& \int_{0}^{1/2}(1-2\cdot \quant)\xq{\quant}d\quant = \int_{0}^{1/2}(1-2\cdot \quant)\frac{1-(1-\quant)^n}{\quant}d\quant-\frac{1}{2}\int_0^{1/2}(1-2\cdot \quant)d\quant\\
\geq~& \int_{0}^{1/2}(1-2\quant)\frac{1-e^{-n \quant}}{\quant}d\quant-\frac{1}{8}\\
=~& \log(n)+\frac{2 \left(1-e^{-\frac{n}{2}}\right)}{n}+\Gamma \left(0,\frac{n}{2}\right)+\gamma -1-\log (2)-\frac{1}{8}\\
\geq~& \log(n)+\gamma -\frac{9}{8}-\log (2) = \Theta(\log(n))
\end{align*}
where $\gamma\approx .57$ is the Euler-Mascheroni constant and $\Gamma \left(0,\frac{n}{2}\right)=\int_{n/2}^{\infty}\frac{e^{-t}}{t}dt\rightarrow 0$.

On the other hand we note that the maximum social welfare achievable by any mechanism that uses $m$ badges is at most 
$n\cdot (m-1)$. For any bid profile $b$, the social welfare from any badge mechanism with $m$ badges is simply:
\begin{equation}
\sum_{t=1}^{m} |i: r_i(b)=t|\left(\frac{n}{|i: r_i(b)\geq t|}-1\right)\leq \sum_{t=1}^{m} n- \sum_{t=1}^{m} |i: r_i(b)=t|= n\cdot m-n
\end{equation}
Therefore, it trivially follows that the optimal revenue achievable with $m$ badges is at most $n\cdot (m-1)$. Thus as 
$n\rightarrow \infty$ the approximation to the optimal revenue achievable with $m$ badges grows as $O\left(\frac{\log(n)}{m-1}\right)$.
\end{example}

To complement the latter example we show that if the mechanism designer sets $\log(n+1)$ badges in a particular way, then the expected total output produced by agents is at least a fourth of the total output in the optimal mechanism. Thereby, a logarithmic number of badges is not only necessary but is also sufficient for a constant approximation. Our analysis makes use of the fact that revenue is equal to expected virtual welfare. We achieve our main result by discarding players with quantile higher than $1/2$ can only lose at most $1/2$ of the optimal revenue and then by constructing a set of $\log(n) + 1$ badges such that each player's status value is at least half of their status value in the optimal mechanism if his quantile is less than $1/2$, thereby approximating the virtual welfare of the optimal mechanism that discards players with quantile higher than $1/2$. 

%We start our analysis by reminding to the reader the revenue equivalence principle: if two mechanisms induce the same interim allocation function at equilibrium
%then their revenue is the same. In fact, to achieve our result we will use an approximate version of the latter principle: if a mechanism at equilibrium induces
%an interim allocation function that is always at least a constant fraction of the interim allocation of the some other mechanism, then the revenue of 
%the first mechanism is a constant fraction of the revenue of the second mechanism, assuming that both mechanisms allocate only
%to non-negative virtual value players. 

%We achieve our main result by showing constructively that there exists a way of setting the thresholds of a logarithmic number of badges, such that
%the interim allocation of any player and for any ability $v_i$, at the unique Bayes-Nash equilibrium is always at least $\left(1-\frac{1}{e}\right)$ of her interim allocation under the optimal ranking mechanism.

To get our result we first give a more general result for arbitrary convex status value functions:
\begin{theorem}\label{thm:general-function}
For any convex status function the badge mechanism with $m=\log\left(\frac{\stat{0}}{\statn{n}{\min\{\tqstar,1/2\}}}\right)\leq \log\left(\frac{\stat{0}}{\statn{n}{1/2}}\right)\leq \log\left(\frac{\stat{0}}{\stat{1/2}}\right)$ badges, such that:
\begin{align*}
\statn{n}{\tq{m}}=~&\frac{\statn{n}{0}}{2}=\frac{\stat{0}}{2}\\
\forall t\in[2, m-1]: \statn{n}{\tq{t}}=~& \frac{\statn{n}{\tq{t+1}}}{2}=\frac{\stat{0}}{2^{m-t+1}}\\
\tq{1}=~ \min\left\{\tqstar,\frac{1}{2}\right\}
\end{align*}
 achieves achieves a $4$-approximation to the total contribution of the optimal mechanism.
\end{theorem}
\begin{proof}
By Equation \eqref{eqn:badge-interim} and by the definition of the contribution thresholds, for any $\quant \in (\tq{t+1},\tq{t}]: \xq{\quant}=\statn{n}{\tq{t}}\geq \frac{\statn{n}{\quant}}{2}$. Additionally, since the badge mechanism assigns positive allocation only to positive virtual value players (i.e. $q\leq \tqstar$), we get:
\begin{equation*}
APX = n\cdot \int_0^{\min\{\tqstar,1/2\}} R'(\quant) \cdot \xq{\quant}d\quant\geq \frac{1}{2}\cdot n\cdot \int_0^{\min\{\tqstar,1/2\}} R'(\quant) \cdot \statn{n}{\quant}d\quant
\end{equation*} 

On the other hand the optimal mechanism achieves total contribution:
\begin{equation*}
OPT = n\cdot \int_0^{\tqstar} R'(\quant)\cdot \xq{\quant}d\quant 
\end{equation*}
If $\tqstar\leq 1/2$, the theorem follows. If $\tqstar >1/2$, then we simply observe that since $R'(\cdot)$ and $\xq{\cdot}$ are both non-increasing functions of the quantile, 
we have:
\begin{equation*}
\int_0^{1/2}R'(\quant)\cdot \xq{\quant} d\quant \geq \int_{1/2}^{\tqstar}R'(\quant)\cdot \xq{\quant}d\quant
\end{equation*} 
and thereby:
\begin{equation*}
OPT \leq 2\cdot n\cdot  \int_0^{1/2}R'(\quant)\cdot \xq{\quant} d\quant \leq 4 \cdot APX
\end{equation*}
\end{proof}

By observing that for the case of $\stat{t} =\frac{n}{(n-1)t+1}-1$, it holds that $\stat{0}=n-1$ and $\stat{1/2}=\frac{n-1}{n+1}$ we get the following corollary.
\begin{corollary}\label{thm:inversely}
If $\stat{t} =\frac{n}{(n-1)t+1}-1$, a badge mechanism with $\log(n+1)$, achieves a $4$-approximation to the optimal contribution.
\end{corollary}
Figure \ref{fig:optimal} portrays the relation between the optimal and the badge interim allocation probabilities for the case of $\stat{t} =\frac{n}{(n-1)t+1}-1$.
\begin{figure}[htpb]
\centering
\includegraphics{optimal-approx.eps}
\caption{Optimal (dashed) versus badge mechanism (solid) interim allocation probabilities, with respect to quantiles.}\label{fig:optimal}
\end{figure}
%\vsdelete{Using similar analysis we can also show that the transition to approximate optimality is smooth. That is if the designer uses $m=\frac{\log{n}}{c}+1$ badges
%then there exists a badge mechanism that achieves a $2^{c}$ approximation. This can be achieved by setting quantile thresholds of the form
%$(\tqstar,\frac{\tqstar}{t},\frac{\tqstar}{t^2},\ldots,\frac{\tqstar}{t^{m-1}})$, for $t=2^{\frac{\log(n)}{m-1}}=2^{c}$.}


==> convex-many_copy.tex <==
% !TEX root=badges.tex 

The previous examples demonstrate the limitations of mechanisms that use a single threshold. With a single threshold, no mechanism can achieve better than a 2-approximation for concave or linear status. Furthermore, no finite approximation is possible for convex status valuations with any constant number of thresholds. We now characterize the approximate optimality of mechanisms with $m > 1$ thresholds. For concave status, the contributions generated by badge mechanism with $m$ badges quickly approaches the contributions of the optimal mechanism. 



\begin{theorem}\label{thm:many-badge-concave}
If the social status function $\stat{\cdot}$ is concave, then a badge mechanism with $m$ badges, can achieve a $\frac{m}{m-2}$-approximation to the total contribution of the optimal mechanism. 
\end{theorem}


For convex valuations, we show that a 4-approximation is possible if the mechanism uses a number of thresholds that is logarithmic in a natural parameter of the status valuation function: $H = \frac{\stat{0}}{\stat{\frac{1}{2}}}$, i.e. the ratio of the status value of the highest ranked user to the status value of a median-ranked user. The next theorem shows that $\log(H)$ badges are sufficient for achieving a constant approximation. For a large class of natural status valuations, this ratio $H$ will be on the order $O(n)$, the number of users. For example, if we use the status value function $\stat{t} =\frac{n}{(n-1)t+1}-1$ from example \ref{convexLowerBound}, then $\stat{0} = n-1$ and $\stat{\frac{1}{2}} = \frac{n-1}{n+1}$ and hence a badge mechanism with $\log(H) = \log(n+1)$ thresholds yields a 4-approximation to the optimal mechanism. Thus the number of necessary thresholds grows slowly with the number of users. 

\begin{theorem}\label{thm:many-badge-convex}
Let $\stat{\cdot}$ be any convex status function and let $\lambda = \min\{ \tqstar ,\frac{1}{2}\}$. The badge mechanism with quantile thresholds $\tqvec=(\tq{1},\ldots,\tq{m})$,  where $m= \log\left(\frac{\stat{0}}{\statn{n}{\lambda}}\right)\leq \log(H)$ and $\tqvec$ satisfies the following:
\begin{align*}
\statn{n}{\tq{m}}= & ~ \frac{\stat{0}}{2}\\
\statn{n}{\tq{t}} = & ~ \frac{ \statn{n}{\tq{t+1}}}{2} = \frac{\stat{0}}{2^{m-t+1}} \qquad  \forall t\in[2, m-1] \\
\tq{1}= & ~ \lambda
\end{align*}
achieves a $4$-approximation to the total contribution of the optimal mechanism. 
\end{theorem}

%\begin{proof}
%
%We will show that the interim status allocation of a user with quantile $\quant < \frac{1}{2}$ in this badge mechanism is at least half of his interim status allocation in the optimal mechanism. This property does not hold for $\quant > \frac{1}{2}$ but we prove that the optimal mechanism generates at most half of its contributions from users with $q > \frac{1}{2}$. The 4-approximation result follows.
%
%By proposition \ref{eqn:badge-interim}, we know that any $\quant < \tqstar$ has an interim status allocation of $\statn{n}{q}$ in the optimal mechanism. We first claim that for any user with with $\quant \in (\tq{t+1},\tq{t}]$ then  $\xq{\quant} \geq \frac{\statn{n}{\quant}}{2}$, i.e. receives at least half of the interim status allocation as the optimal mechanism. Any user with $\quant \in (\tq{t+1},\tq{t}]$ receives an interim status allocation of $ \xq{\quant} = \xq{\tq{t}} = \statn{n}{\tq{t}}$ in this badge mechanism. By the design of the thresholds, $\statn{n}{\tq{t}} = \frac{\statn{n}{\tq{t+1}}}{2} \geq  \frac{\statn{n}{q}}{2}$ where the last inequality follows because $\statn{n}{\cdot}$ is decreasing in quantile and $q > \tq{t+1}$. 
%
%Since this mechanism assigns non-zero status value only to users with $q\leq \tqstar$ and $\xq{\quant} \geq \frac{\statn{n}{\quant}}{2}$ we get:
%\begin{equation*}
%APX =  \int_0^{\min\{\tqstar,1/2\}} R'(\quant) \cdot \xq{\quant}d\quant\geq \frac{1}{2}\cdot \int_0^{\min\{\tqstar,1/2\}} R'(\quant) \cdot \statn{n}{\quant}d\quant
%\end{equation*} 
%
%\noindent On the other hand the optimal mechanism achieves total contribution:
%\begin{equation*}
%OPT = \int_0^{\tqstar} R'(\quant)\cdot \statn{n}{\quant} d\quant 
%\end{equation*}
%If $\tqstar\leq 1/2$, then we get $2 \cdot APX \geq OPT$. 
%
%
%If $\tqstar >1/2$, then:
%\begin{equation*}
%OPT = \int_0^{1/2}R'(\quant)\cdot \xq{\quant} d\quant +  \int_{1/2}^{\tqstar}R'(\quant)\cdot \xq{\quant}d\quant
%\end{equation*}
%$R'(\cdot)$ and $\xq{\cdot}$ are both non-increasing functions of the quantile, so the following inequality holds: 
%\begin{equation*}
%\int_0^{1/2}R'(\quant)\cdot \xq{\quant} d\quant \geq \int_{1/2}^{\tqstar}R'(\quant)\cdot \xq{\quant}d\quant
%\end{equation*} 
%and thereby:
%\begin{equation*}
%OPT \leq 2\cdot  \int_0^{1/2}R'(\quant)\cdot \xq{\quant} d\quant \leq 4 \cdot APX
%\end{equation*}
%\end{proof}




==> equilibrium.tex <==
% !TEX root = badges.tex

\begin{proofof}{Theorem \ref{thm:uniqueness}}
We start by observing that if a player gets status class $r_i$, her output should be exactly the threshold to win that badge, $\tb{r_i}$,  because producing more output would cost more effort and would not increase her value. Additionally, it is easy to see that the equilibrium mapping would be monotone in quantile, i.e. if $\quant[1]>\quant[2]$ then $b(\quant[1])\leq b(\quant[2])$. In other words if a player with quantile $\quant[1]$ bids $\tb{r_1}$ and with value $\quant[2]<\quant[1]$ he bids $\tb{r_2}$ then it must be that $r_1\leq r_2$. \footnote{Suppose the contrary. For simplicity, denote with $x_{r}$ the expected status that a player gets from bidding $\tb{r}$, assuming the rest of the players follow strategy $b(\cdot)$. Since, $r_1>r_2$ we have $\tb{r_1}> \tb{r_2}$. Since $b(\quant[1])$ is an equilibrium for a player with value $\quant[1]$, it must be that $\val(\quant[1]) (x_{r_1}-x_{r_2})\geq \tb{r_1}-\tb{r_2}>0$. Thus $x_{r_1}>x_{r_2}$ and since $\val(\quant[2])>\val(\quant[1])$ we get: $\val(\quant[2])(x_{r_1}-x_{r_2})>\val(\quant[1])(x_{r_1}-x_{r_2})\geq  \tb{r_1}-\tb{r_2}$. But the latter implies, $\val(\quant[2])\cdot  x_{r_1} -\tb{r_1}>\val(\quant[2])\cdot x_{r_2}-\tb{r_2}$ and 
therefore $b(\val[2])$ cannot be an equilibrium for a player with quantile $\quant[2]$.}


Since the equilibrium mapping is a monotone step function of quantile, it is defined by a set of thresholds in the quantile space $\tq{1},\ldots,\tq{p}$, for some $p\leq m$, such that if player $i$ has quantile $\quant[i]\in (\tq{t+1},\tq{t}]$ then he produces output $b(\quant[i])=\tb{t}$. If $\quant[i] >\tq{1}$ then $b(\quant[i])=0$ and if $\quant[i] \leq \tq{p}$ then
$b(\quant[i])=\tb{p}$. For notational convenience we will denote with $\tq{0}=1$ and $\tq{p+1}=0$. Observe that it is not necessarily true that $p=m$, since some contribution thresholds might be too high.

To characterize the BNE, it remains to compute those quantile thresholds and show that they are unique. A player's status value is a function of the proportion of other players with a weakly better badge. A player with quantile $\quant[i]\in [\tq{t+1},\tq{t}]$ earns the badge associated with quantile $\tq{t}$; thus, because the equilibrium is a monotone step function, any player that has a quantile less than $\tq{t}$ will earn a weakly better badge than player i. By definition, a player has a lower quantile than $\tq{t}$ with probability $\tq{t}$. This allows us to compute the interim status value of player $i$ with quantile $\quant[i]\in [\tq{t+1},\tq{t}]$ as: 
\begin{equation}
\xq{\quant[i]} =  \statn{n}{\tq{t}}
\end{equation}
where $\statn{n}{\cdot}$ is given by Equation \eqref{eqn:expectedstatus}. 

By the payment identity of Lemma \ref{lem:myerson-bne}, for the vector of quantiles $\tqvec$ to be an equilibrium they must satisfy the following equation:
\begin{align}\label{eqn:effort-to-value}
\forall t\in[1,\ldots, p]: \tb{t} =\sum_{j=1}^t \val(\tq{j})\cdot \left(\statn{n}{\tq{j}}-\statn{n}{\tq{j-1}}\right)
\end{align}
This relationship is depicted in Figure \ref{fig:interim-characterization}. 
\begin{figure}[htpb]
\centering
\subfigure{\includegraphics[scale=0.7]{bid_equilibrium.eps}}
\subfigure{\includegraphics[scale=0.7]{interim.eps}}
\caption{Equilibrium bid function (left) and relation between interim status allocation and contribution thresholds at equilibrium (right).}\label{fig:interim-characterization}
\end{figure}
Equivalently, the above set of conditions can be re-written as:
\begin{align}\label{eqn:value-to-effort}
\forall t\in [1,\ldots,p]:~& \val(\tq{t})\cdot \left(\statn{n}{\tq{t}}-\statn{n}{\tq{t-1}}\right)=\tb{t}-\tb{t-1}
\end{align} 
This set of equalities has an intuitive interpretation as saying that the players with quantiles at the boundary of two badges should be indifferent between getting either of the two badges. Additionally, to ensure that the latter is an equilibrium we also need to make sure that if $p<m$, then the highest ability player doesn't prefer being on badge $p+1$ alone, rather than being on badge $p$:
\begin{align}\label{eqn:value-to-effort-2}
\text{if } p<m:~& \val(0)\cdot \left(\statn{n}{0}-\statn{n}{\tq{p}}\right)\leq \tb{p+1}-\tb{p}
\end{align}
To show uniqueness of the symmetric equilibrium we simply need to show that the above set of conditions have a unique solution.

\begin{lemma}\label{lem:uniqueness} There exists a unique $p\leq m$ and a unique vector $\tqvec=(\tq{1},\ldots,\tq{p})$, that satisfies the system of Equations \eqref{eqn:value-to-effort} and \eqref{eqn:value-to-effort-2}.
\end{lemma}
\begin{proof}
Given a profile of badge thresholds $\tbvec$, we show recursively that there is a unique set of quantile thresholds which satisfies the set of equations. For $t=1$, Equation \eqref{eqn:value-to-effort} becomes: $\tb{1} = \val(\tq{1})\cdot \statn{n}{\tq{1}}$. Observe that $\val(0)\cdot \statn{n}{0}=\bar{\val}\cdot \stat{0}$, $\val(1)\cdot \statn{n}{1}=0$, $\val(x)\cdot \statn{n}{x}$ is continuous decreasing. If $\tb{1}<\bar{\val}\cdot \stat{0}$ then a unique solution exists (recall that $\bar{\val}$ is the upper bound of the ability distribution). Otherwise, no player is willing to bid as high as $\tb{1}$ (or any $\tb{t}$ for $t>1$) and the recursion stops with $p=0$. Subsequently, find the solution $\tv{2}$ to the equation: $\tb{2}-\tb{1}= \val(\tq{2}) (\statn{n}{\tq{2}} - \statn{n}{\tq{1}})$. For similar reason, either a unique such solution exists or no player (not even a player with ability $\bar{\val}$) is willing to bid $\tb{2}$ rather than bid $\tb{1}$ and we can stop the recursion, setting $p=1$. Then solve for $\tq{3},\ldots, \tq{p}$ in the same way.
\end{proof}
The latter Lemma completes the proof of the uniqueness and characterization of the equilibrium. The inverse part of the theorem, is trivial based on the previous discussion. 
\end{proofof}

%\footnote{A similar analysis can be achieved for distributions with bounded support, but one should simply disregard badge thresholds that pass the upper bound of the distribution of player's ability.}.
%
%Lemma \ref{lem:uniqueness} establishes that for any given set of contribution thresholds, the symmetric Bayes-Nash equilibrium is unique. An equivalent way of phrasing the equilibrium conditions in Equation \eqref{eqn:value-to-effort} is:
%\begin{align}\label{eqn:effort-to-value}
%\forall t\in[1,\ldots, p]: \tb{t} =\sum_{j=1}^t \val(\tq{j})\cdot \left(\statn{n}{\tq{j}}-\statn{n}{\tq{t-1}}\right)
%\end{align}
% An alternative way of showing that this relationship must be satisfied at equilibrium is by invoking Myerson's \cite{myerson81} equilibrium characterization to our setting. 
%\begin{figure}[htpb]
%\subfigure{\includegraphics[scale=0.7]{bid_equilibrium.eps}}
%\subfigure{\includegraphics[scale=0.7]{interim.eps}}
%\caption{Equilibrium bid function (left) and relation between interim status allocation and contribution thresholds at equilibrium (right).}\label{fig:interim-characterization}
%\end{figure}
%The latter equation portrays that if instead of the contribution thresholds, we are given a vector of target quantile thresholds
%$\tqvec=(\tq{1},\ldots,\tq{p})$, then we can always find a set of contribution thresholds, such that the unique BNE is characterized by quantile thresholds $\tqvec$. 
%
%%The following corollary of the above discussion summarizes a property that will prove very useful in subsequent sections: 
%
%\vscomment{The following should be obsolete by this point.}
%\textbf{Optimal Design in Quantile Space.} The main implication of Theorem \ref{thm:uniqueness} is that instead of setting contribution thresholds, a designer could optimize over thresholds in the quantile space and then compute the badges needed to implement the ability thresholds. This formulation of the problem is easier because we no longer need to worry about the induced equilibrium behavior. For the remainder of the paper, we focus on this version of the problem. Observe that by setting a set of quantile thresholds $\tqvec$, essentially the designer sets a set of target congestions of each badge, since the expected proportion of players that will get badge $t$ will be equal to $\kappa_{t}-\kappa_{t+1}$. Intuitively, the optimal design of badges boils down to the optimal design of equilibrium badge congestions.
%
%Using the equilibrium characterization we can also compute the expected revenue produced by a set of badges with thresholds $\tqvec=(\tq{1},\ldots,\tq{m})$ in the quantile space as follows: If a player has quantile $\quant[i]\in (\tq{t+1},\tq{t}]$ then by Equation
%\eqref{eqn:effort-to-value} we get that he submits a bid of $\tb{t}=\sum_{j=1}^t \val(\tq{j})\cdot \left(\statn{n}{\tq{j}}-\statn{n}{\tq{t-1}}\right)$. The latter happens with probability $\tq{t} - \tq{t+1}$. Thus a player's expected payment, after some rearrangements, is:
%\begin{align*}
%\E_{\quant[i]}[b(\quant[i])] =\sum_{t=1}^m (\tq{t}-\tq{t+1})\cdot \tb{t}
%= \sum_{t=1}^m \tq{t}\cdot (\tb{t}-\tb{t-1})
%%=~& \sum_{t=1}^m  \left(v(\kappa_t)\left(\hat{x}(\kappa_t)-\hat{x}(\kappa_{t-1})\right) \sum_{j=t}^m  (\kappa_j-\kappa_{j+1})\right)\\
%%=~& \sum_{t=1}^m  v(\kappa_t)\left(\hat{x}(\kappa_t)-\hat{x}(\kappa_{t-1})\right)(\kappa_t - \kappa_{m+1})\\
%=~& \sum_{t=1}^m \kappa_t \cdot \val(\kappa_t)\cdot \left(\statn{n}{\kappa_t}-\statn{n}{\kappa_{t-1}}\right)
%\end{align*}
%Let $R(x)=\val(x)\cdot x$, which is usually denoted as the revenue function of the distribution \cite{Bulow1989,Hartline2012}, since it corresponds to the revenue of a monopolist,
%facing a single buyer and posting a price such that he sells with probability $x$.Thus the total revenue of the mechanism is simply:
%\begin{align}
%\E\left[\sum_i b_i(\quant[i])\right] = ~& n \cdot 
% \sum_{t=1}^m R(\tq{t})\cdot \left(\statn{n}{\tq{t}}-\statn{n}{\tq{t-1}}\right)\label{eqn:badge-mechanism-rev-1}\\
%= ~& n \cdot 
% \sum_{t=1}^m \left(R(\tq{t})-R(\tq{t+1})\right)\cdot\statn{n}{\tq{t}}\label{eqn:badge-mechanism-rev-2}
%\end{align}










==> equilibrium.tex.old.tex <==
% !TEX root = badges.tex

\subsection{Equilibrium of Multi-Level Absolute Threshold Badges}
We begin our analysis by characterizing the Bayes-Nash equilibria of any badge mechanism with contribution thresholds $\theta_1,\ldots,\theta_m$. We focus on symmetric equilibria\footnote{We note that asymmetric equilibria do exist in our setting, even in the case of a single badge and two players distributed $U[0,1]$.} and show there is a unique symmetric equilibrium. This equilibrium is monotone, non-increasing in each player's quantile. Recall that a lower quantile implies a higher ability, so the higher ability players will contribute more than lower ability players in this equilibrium. 
%
% which is monotone, i.e. each player uses the same strategy mapping $b_i(\quant[i]) = b(\quant[i])$ and this mapping is monotone non-increasing in the player's quantile. More generally, the purpose of this section is to show the following theorem.

\begin{theorem}\label{thm:uniqueness}
Every vector of contribution thresholds $\tbvec=(\tb{1},\ldots,\tb{m})$ has a unique symmetric BNE characterized by quantile thresholds $\tqvec=(\tq{1},\ldots,\tq{p})$ for some $p\leq m$, such that $b(\quant[i])=\theta_t$ if $\quant[i]\in (\tq{t+1},\tq{t}]$. Moreover, for any vector of quantile thresholds $\tqvec=(\tq{1},\ldots, \tq{p})$ there exists a set of contribution thresholds under which the unique symmetric BNE is characterized by $\tqvec$.
\end{theorem}

We start by observing that if a player gets status class $r_i$, her output should be exactly the threshold to win that badge, $\tb{r_i}$,  because producing more output would cost more effort and would not increase her value. Additionally, it is easy to see that the equilibrium mapping would be monotone in quantile, i.e. if $\quant[1]>\quant[2]$ then $b(\quant[1])\leq b(\quant[2])$. In other words if 
a player with quantile $\quant[1]$ bids $\tb{r_1}$ and with value $\quant[2]<\quant[1]$ he bids $\tb{r_2}$ then it must be that
$r_1\leq r_2$. \footnote{Suppose the contrary. For simplicity, denote with $x_{r}$ the expected status that a player gets from 
bidding $\tb{r}$, assuming the rest of the players follow strategy $b(\cdot)$. Since, $r_1>r_2$ we have $\tb{r_1}> \tb{r_2}$. Since $b(\quant[1])$ is an equilibrium for a player with value $\quant[1]$, it must be that $\val(\quant[1]) (x_{r_1}-x_{r_2})\geq \tb{r_1}-\tb{r_2}>0$.
Thus $x_{r_1}>x_{r_2}$ and since $\val(\quant[2])>\val(\quant[1])$ we get: $\val(\quant[2])(x_{r_1}-x_{r_2})>\val(\quant[1])(x_{r_1}-x_{r_2})\geq  \tb{r_1}-\tb{r_2}$. But the latter implies, $\val(\quant[2])\cdot  x_{r_1} -\tb{r_1}>\val(\quant[2])\cdot x_{r_2}-\tb{r_2}$ and 
therefore $b(\val[2])$ cannot be an equilibrium for a player with quantile $\quant[2]$.}


Since the equilibrium mapping is a monotone step function of quantile, it is defined by a set of thresholds in the quantile space $\tq{1},\ldots,\tq{p}$, for some $p\leq m$, such that if player $i$ has quantile $\quant[i]\in (\tq{t+1},\tq{t}]$ then he produces output $b(\quant[i])=\tb{t}$. If $\quant[i] >\tq{1}$ then $b(\quant[i])=0$ and if $\quant[i] \leq \tq{p}$ then
$b(\quant[i])=\tb{p}$. For notational convenience we will denote with $\tq{0}=1$ and $\tq{p+1}=0$. Observe that it is not necessarily true that $p=m$, since some contribution thresholds might be too high.

To characterize the BNE, it remains to compute those quantile thresholds and show that they are unique. A player's status value is a function of the proportion of other players with a weakly better badge. A player with quantile $\quant[i]\in [\tq{t+1},\tq{t}]$ earns the badge associated with quantile $\tq{t}$; thus, because the equilibrium is a monotone step function, any player that has a quantile less than $\tq{t}$ will earn a weakly better badge than player i. By definition, a player has a lower quantile than $\tq{t}$ with probability $\tq{t}$. This allows us to compute the interim status value of player $i$ with quantile $\quant[i]\in [\tq{t+1},\tq{t}]$ as: 
\begin{equation}
\xq{\quant[i]} =  \statn{n}{\tq{t}}
\end{equation}
where $\statn{n}{\cdot}$ is given by Equation \eqref{eqn:badge-interim}. 

By Lemma \ref{lem:myerson}, for the vector of quantiles $\tqvec$ to be an equilibrium they must satisfy the following equation:
\begin{align}\label{eqn:effort-to-value}
\forall t\in[1,\ldots, p]: \tb{t} =\sum_{j=1}^t \val(\tq{j})\cdot \left(\statn{n}{\tq{j}}-\statn{n}{\tq{j-1}}\right)
\end{align}
This relationship is depicted in Figure \ref{fig:interim-characterization}. 
\begin{figure}[htpb]
\centering
\subfigure{\includegraphics[scale=0.7]{bid_equilibrium.eps}}
\subfigure{\includegraphics[scale=0.7]{interim.eps}}
\caption{Equilibrium bid function (left) and relation between interim status allocation and contribution thresholds at equilibrium (right).}\label{fig:interim-characterization}
\end{figure}
Equivalently, the above set of conditions can be re-written as:
\begin{align}\label{eqn:value-to-effort}
\forall t\in [1,\ldots,p]:~& \val(\tq{t})\cdot \left(\statn{n}{\tq{t}}-\statn{n}{\tq{t-1}}\right)=\tb{t}-\tb{t-1}
\end{align} 
This set of equalities has an intuitive interpretation as saying that the players with quantiles at the boundary of two badges should be indifferent between getting either of the two badges. Additionally, to ensure that the latter is an equilibrium we also need to make sure that if $p<m$, then the highest ability player doesn't prefer being on badge $p+1$ alone, rather than being on badge $p$:
\begin{align}\label{eqn:value-to-effort-2}
\text{if } p<m:~& \val(0)\cdot \left(\statn{n}{0}-\statn{n}{\tq{p}}\right)\leq \tb{p+1}-\tb{p}
\end{align}
To show uniqueness of the symmetric equilibrium we simply need to show that the above set of conditions have a unique solution.

\begin{lemma}\label{lem:uniqueness} There exists a unique $p\leq m$ and a unique vector $\tqvec$, that satisfies the system of Equations \eqref{eqn:value-to-effort} and \eqref{eqn:value-to-effort-2}.
\end{lemma}
\begin{proof}
Given a profile of badge thresholds $\tbvec$, we show recursively that there is a unique set of quantile thresholds which satisfies the set of equations. For $t=1$, Equation \eqref{eqn:value-to-effort} becomes: $\tb{1} = \val(\tq{1})\cdot \statn{n}{\tq{1}}$. Observe that $\val(0)\cdot \statn{n}{0}=\bar{\val}\cdot \stat{0}$, $\val(1)\cdot \statn{n}{1}=0$, $\val(x)\cdot \statn{n}{x}$ is continuous decreasing. If $\tb{1}<\bar{\val}\cdot \stat{0}$ then a unique solution exists (recall that $\bar{\val}$ is the upper bound of the ability distribution). Otherwise, no player is willing to bid as high as $\tb{1}$ (or any $\tb{t}$ for $t>1$) and the recursion stops with $p=0$. Subsequently, find the solution $\tv{2}$ to the equation: $\tb{2}-\tb{1}= \val(\tq{2}) (\statn{n}{\tq{2}} - \statn{n}{\tq{1}})$. For similar reason, either a unique such solution exists or no player (not even a player with ability $\bar{\val}$) is willing to bid $\tb{2}$ rather than bid $\tb{1}$ and we can stop the recursion, setting $p=1$. Then solve for $\tq{3},\ldots, \tq{p}$ in the same way.
\end{proof}
%\footnote{A similar analysis can be achieved for distributions with bounded support, but one should simply disregard badge thresholds that pass the upper bound of the distribution of player's ability.}.
%
%Lemma \ref{lem:uniqueness} establishes that for any given set of contribution thresholds, the symmetric Bayes-Nash equilibrium is unique. An equivalent way of phrasing the equilibrium conditions in Equation \eqref{eqn:value-to-effort} is:
%\begin{align}\label{eqn:effort-to-value}
%\forall t\in[1,\ldots, p]: \tb{t} =\sum_{j=1}^t \val(\tq{j})\cdot \left(\statn{n}{\tq{j}}-\statn{n}{\tq{t-1}}\right)
%\end{align}
% An alternative way of showing that this relationship must be satisfied at equilibrium is by invoking Myerson's \cite{myerson81} equilibrium characterization to our setting. 
%\begin{figure}[htpb]
%\subfigure{\includegraphics[scale=0.7]{bid_equilibrium.eps}}
%\subfigure{\includegraphics[scale=0.7]{interim.eps}}
%\caption{Equilibrium bid function (left) and relation between interim status allocation and contribution thresholds at equilibrium (right).}\label{fig:interim-characterization}
%\end{figure}
%The latter equation portrays that if instead of the contribution thresholds, we are given a vector of target quantile thresholds
%$\tqvec=(\tq{1},\ldots,\tq{p})$, then we can always find a set of contribution thresholds, such that the unique BNE is characterized by quantile thresholds $\tqvec$. 
%
%%The following corollary of the above discussion summarizes a property that will prove very useful in subsequent sections: 
%
%\vscomment{The following should be obsolete by this point.}
%\textbf{Optimal Design in Quantile Space.} The main implication of Theorem \ref{thm:uniqueness} is that instead of setting contribution thresholds, a designer could optimize over thresholds in the quantile space and then compute the badges needed to implement the ability thresholds. This formulation of the problem is easier because we no longer need to worry about the induced equilibrium behavior. For the remainder of the paper, we focus on this version of the problem. Observe that by setting a set of quantile thresholds $\tqvec$, essentially the designer sets a set of target congestions of each badge, since the expected proportion of players that will get badge $t$ will be equal to $\kappa_{t}-\kappa_{t+1}$. Intuitively, the optimal design of badges boils down to the optimal design of equilibrium badge congestions.
%
%Using the equilibrium characterization we can also compute the expected revenue produced by a set of badges with thresholds $\tqvec=(\tq{1},\ldots,\tq{m})$ in the quantile space as follows: If a player has quantile $\quant[i]\in (\tq{t+1},\tq{t}]$ then by Equation
%\eqref{eqn:effort-to-value} we get that he submits a bid of $\tb{t}=\sum_{j=1}^t \val(\tq{j})\cdot \left(\statn{n}{\tq{j}}-\statn{n}{\tq{t-1}}\right)$. The latter happens with probability $\tq{t} - \tq{t+1}$. Thus a player's expected payment, after some rearrangements, is:
%\begin{align*}
%\E_{\quant[i]}[b(\quant[i])] =\sum_{t=1}^m (\tq{t}-\tq{t+1})\cdot \tb{t}
%= \sum_{t=1}^m \tq{t}\cdot (\tb{t}-\tb{t-1})
%%=~& \sum_{t=1}^m  \left(v(\kappa_t)\left(\hat{x}(\kappa_t)-\hat{x}(\kappa_{t-1})\right) \sum_{j=t}^m  (\kappa_j-\kappa_{j+1})\right)\\
%%=~& \sum_{t=1}^m  v(\kappa_t)\left(\hat{x}(\kappa_t)-\hat{x}(\kappa_{t-1})\right)(\kappa_t - \kappa_{m+1})\\
%=~& \sum_{t=1}^m \kappa_t \cdot \val(\kappa_t)\cdot \left(\statn{n}{\kappa_t}-\statn{n}{\kappa_{t-1}}\right)
%\end{align*}
%Let $R(x)=\val(x)\cdot x$, which is usually denoted as the revenue function of the distribution \cite{Bulow1989,Hartline2012}, since it corresponds to the revenue of a monopolist,
%facing a single buyer and posting a price such that he sells with probability $x$.Thus the total revenue of the mechanism is simply:
%\begin{align}
%\E\left[\sum_i b_i(\quant[i])\right] = ~& n \cdot 
% \sum_{t=1}^m R(\tq{t})\cdot \left(\statn{n}{\tq{t}}-\statn{n}{\tq{t-1}}\right)\label{eqn:badge-mechanism-rev-1}\\
%= ~& n \cdot 
% \sum_{t=1}^m \left(R(\tq{t})-R(\tq{t+1})\right)\cdot\statn{n}{\tq{t}}\label{eqn:badge-mechanism-rev-2}
%\end{align}










==> experimental.tex <==
% !TEX root=badges.tex

We will analyze the optimality of stack overflow badges from the perspective of our utility model and our equilibrium analysis. Our data set consists of a set of badge thresholds, together with the congestion of each badge. We will work mainly with moderation badges. 
An example of such a badge is associated with the task of raising helpful moderation flags on posted questions. Stack overflow has a three-level badge for this task, where a player is awarded the first badge if he raises one flag, the second badge for raising $80$ helpful flags and the third badge for raising $500$ helpful flags. Additionally, we know the congestion of each badge, i.e. $60.2k$ 
people have been awarded the first badge, $2.9k$ people the second badge and $619$ people the third one.  

Observe that such a badge falls withing our model, where we assume that each player has some ability $v_i$ for raising helpful flags, and if he invests some amount of time $e_i$ he will produce an amount of helpful flags of $v_i\cdot e_i$, while he will incur a cost of $e_i$.

Our analysis will proceed as follows: we will first assume that the distribution of abilities comes from some reasonable class of parameterized distributions, e.g. normal, exponential etc., with unknown parameters. Assuming that players are playing at the Bayes-Nash equilibrium for this distribution, we know that the congestions of each badge will be the ones predicted at the equilibrium described in Section \ref{sec:equilibrium}. Specifically, if the badge thresholds $\theta=(\theta_1,\ldots,\theta_m)$, under a common belief of ability distribution $F$, induced an equilibrium with ability thresholds $a=(a_1,\ldots,a_m)$, then the expected congestion at badge $j$ will be $n\cdot (F(a_j)-F(a_{j-1}))$. Thus by knowing the actual congestion $n_j$ and assuming that $n$ is large enough such that assuming that the expected congestion occurs is not a bad approximation, we can infer the CDF of the distribution at
the ability thresholds, i.e. :
\begin{equation}
F(a_j) = \frac{1}{n}\sum_{t\leq j}n_j
\end{equation}
Additionally, from the equilibrium characterization we can infer the expected allocation of each player at equilibrium, 
\begin{equation}
\tilde{x}(a_j) = \frac{1-F(a_j)^n}{n(1-F(a_j))}=\frac{1- \left(\frac{1}{n}\sum_{t\leq j}n_j\right)^n}{n-\sum_{t\leq j}n_j}=\frac{1- \left(\frac{1}{n}\sum_{t\leq j}n_j\right)^n}{\sum_{t> j}n_j}
\end{equation}
Last from the equilibrium characterization, we can also infer the actual ability threshold $a_j$ as follows:
\begin{equation}
a_j = \frac{\theta_j-\theta_{j-1}}{\tilde{x}(a_j)-\tilde{x}(a_{j-1})}
\end{equation}
Having the pairs $(a_j,F(a_j))_{j\in[m]}$, we can then fit the parameters of the class of distributions that we assumed and infer the distribution of abilities. Using the inferred distribution of abilities, we can actually compute the optimal vector of $m$ badge thresholds and compare it with the vector of used badge thresholds.



==> extensions.tex <==
% !TEX root=badges.tex


\subsection{Addition of Badges and Revenue Monotonicity}
A natural question is whether an extra badge at some prefixed quantile threshold can actually hurt revenue. We
show that this cannot happen as long as the quantile threshold of this extra badge is above the monopoly quantile of the distribution. 

\begin{lemma}Adding an extra badge with quantile threshold $\tilde{\kappa}\geq \kappa^*$ can only increase the revenue of an existing
badge mechanism. 
\end{lemma}
\begin{proof}
%The revenue of badge mechanism with quantile thresholds $\kappa=(\kappa_1,\ldots,\kappa_m)$ can be rewritten as:
%\begin{equation}
%REV_{\kappa}=\sum_{t=1}^{m}(R(\kappa_t)-R(\kappa_{t+1}))\cdot \hat{x}(\kappa_t)
%\end{equation}
%where we assumed that $\kappa_{m+1}=0$ and hence $R(\kappa_{m+1})=0$.
Consider augmenting the badge mechanism with an extra badge with quantile threshold $\tilde{\kappa}$ and such that $\tilde{\kappa}\in [\kappa_{t+1},\kappa_t]$ for some $t\in [1,m]$, with the convention that $\kappa_{m+1}=0$ and $\kappa_{0}=1$. Then the revenue of this new mechanism is:
\begin{equation*}
REV_{\kappa+\tilde{\kappa}}=\sum_{\sigma \neq t }(R(\kappa_t)-R(\kappa_{t+1})\cdot \hat{x}(\kappa_t) +(R(\kappa_t)-R(\tilde{\kappa}))\cdot \hat{x}(\kappa_t)+
(R(\tilde{\kappa})-R(\kappa_{t+1}))\cdot \hat{x}(\tilde{\kappa})
\end{equation*}
By regularity of the distribution, we know that $R(\cdot)$ is monotone in the region $[0,\kappa^*]$. Since we assumed that $\tilde{\kappa}\leq \kappa^*$
we get that $R(\tilde{\kappa})\geq R(\kappa_{t+1})$. By monotonicity of $\hat{x}(\cdot)$ we also have: $\hat{x}(\tilde{\kappa})\geq \hat{x}(\kappa_t)$. 
Combining the above we get the Lemma:
\begin{align*}
REV_{\kappa+\tilde{\kappa}}\geq~& \sum_{\sigma \neq t }(R(\kappa_t)-R(\kappa_{t+1})\cdot \hat{x}(\kappa_t) +(R(\kappa_t)-R(\tilde{\kappa}))\cdot \hat{x}(\kappa_t)+
(R(\tilde{\kappa})-R(\kappa_{t+1}))\cdot \hat{x}(\kappa_t)\\
=~&\sum_{\sigma \neq t }(R(\kappa_t)-R(\kappa_{t+1})\cdot \hat{x}(\kappa_t) +(R(\kappa_t)-R(\kappa_{t+1}))\cdot \hat{x}(\kappa_t)=REV_{\kappa}
\end{align*}
\end{proof}

\vsdelete{I think the comparative revenue analysis is not  that compelling, so I removed it.}
%\subsection{Comparative Revenue Analysis} Another interesting direction is which type of status utility leads to higher amount of contribution. We show that under some normalization assumption, optimal revenue is higher in the case of convex status functions than in the case of concave. Intuitively, convex status leads to higher competition and thereby higher contribution.
%
%\begin{theorem} Consider two status functions $S_1(\cdot)$ and $S_2(\cdot)$, such that $S_1(\cdot)$ is convex,
%$S_2(\cdot)$ is concave, $S_1(1)=S_2(1)=0$ and the expected social welfare of the optimal mechanism is identical:
%\begin{equation}
%\int_0^{\tqstar} \val(\quant) \hat{x}_1(\quant)d\quant=\int_0^{\tqstar} \val(\quant) \hat{x}_2(\quant)d\quant
%\end{equation}
%where:
%\begin{equation}
%\hat{x}_r(\quant)=\sum_{\nu=0}^{n-1}S_r\left(\frac{\nu+1}{n}\right)\beta_{n-1, \nu}(\quant)
%\end{equation}
%If the ability distribution satisfies the Monotone Hazard Rate condition, then the optimal revenue under $S_1(\cdot)$
%is higher than the revenue under $S_2(\cdot)$.
%\end{theorem}
%\begin{proof}
%Observe that $\hat{x}_1(\cdot)$ is convex, $\hat{x}_2(\cdot)$ is concave, $\hat{x}_1(1)=\hat{x}_2(1)=0$. Thus there are
%only two cases: 1) either $\hat{x}_1(\cdot)$ lies strictly above $\hat{x}_2(\cdot)$ in the region $[0,1]$ or 2) $\hat{x}_1(\cdot)$
%lies below $\hat{x}_2(\cdot)$ in a region $[t,1]$ and lies above in the region $[0,t]$.
%
%By the equal welfare property:
%\begin{equation}
%\int_0^{\tqstar} \val(\quant) \cdot \left(\hat{x}_1(\quant)-\hat{x}_2(\quant)\right)d\quant=0
%\end{equation}
%Since $\val(\quant)$ is a non-negative function, it must be that only the second case is valid. Thus if we denote with
%$g(q)=\hat{x}_1(\quant)-\hat{x}_2(\quant)$, then $g(q)$ is positive in the region $[0,t]$ and negative in $[t,1]$ and $t\in[0,\tqstar]$.
%
%Since $\val(\quant)$ is decreasing, it is then implied that:
%\begin{equation}\label{eqn:diff-negative}
%\int_0^{\tqstar} g(\quant)d\quant = \int_0^{\tqstar}  \hat{x}_1(\quant)-\hat{x}_2(\quant)d\quant<0
%\end{equation}
%The difference in optimal per-player revenue under the two functions is:
%\begin{align*}
%\E[p_1(\quant)-p_2(\quant)]=~&\int_0^{\tqstar} R'(\quant) g(\quant)d\quant\\
%=~&\int_0^{\tqstar} \val(\quant) \cdot g(\quant) d\quant+\int_0^{\tqstar} q \cdot \val'(\quant) \cdot g(\quant)d\quant\\
%=~&\int_0^{\tqstar} q\cdot \val'(\quant) \cdot g(\quant)d\quant
%\end{align*}
%Since $\val(\quant)$ is decreasing, $-\quant\val'(\quant)\geq 0$. If $-\quant\val'(\quant)$ is increasing, then following
%Equation \eqref{eqn:diff-negative} and the properties of $g(\quant)$ we have:
%\begin{align*}
%\int_0^{\tqstar} (-q\cdot \val'(\quant)) \cdot g(\quant) d\quant<0
%\end{align*}
%since the positive parts of $g(q)$ are amplified less than the negative parts. Thus we get that:
%\begin{align*}
%\E[p_1(\quant)-p_2(\quant)]=\int_0^{\tqstar} q\cdot \val'(\quant) \cdot g(\quant)d\quant>0
%\end{align*}
%\end{proof}

\vsdelete{\vscomment{I vote that we might want to remove the following model, since we now have a general enough status model and this one doesn't fit the general framework that we worked with throughout the paper.}
\subsection{Discounted Externality Model} We consider the utility model where players not only care about how many
people have the same status class as them, but rather discount the negative effect of other bidders according to how far above or below they are. Specifically, if $\delta_j(r)=|\{i\in [n]: r_i=j\}|$ is the number of players with rank $j$ then:
\begin{equation}
\hat{u}_i(r,e_i) = \frac{1}{\sum_{t=1}^{m} \alpha^{t-r_i} \delta_t(r)}-e_i = \frac{\alpha^{r_i}}{\sum_{t=1}^m a^t \delta_t(r)}-e_i
\end{equation}
for some $\alpha\geq 1$. 
Observe that for such utility functions we have that for any allocation of ranks $\sum_i x_i(r) =1$. Thus the auction setting
is equivalent to a mechanism design with one unit for sale. Additionally, the single-badge mechanism with some ability
threshold $a$ corresponds to an auction where the unit is sold uniformly at random to any player with value above the reserve
$a$. By applying a prophet inequality analysis it is known that there exists such a reserve $a$ such that the revenue is at least
half of the optimal single-item auction revenue. 
\begin{theorem} In the discounted externalities utility model, a single badge can achieve half approximation to the optimal
ranking mechanism.
\end{theorem}
}

\subsection{Convex Effort Costs} An interpretation of our model is that if a player wants to contribute $b_i$ then he needs to invest an effort of $\frac{b_i}{\val[i]}$. Then we assumed that a players cost is linear in his effort. However, in many cases cost is a convex function of effort (e.g. soft budget of effort constraints). We consider the following generalization of player utilities that addresses this concern:
\begin{equation}
\hat{u}_i(r,b_i) = x_i(r) - \left(\frac{b_i}{\val[i]}\right)^{\alpha}
\end{equation}
for some $\alpha\geq 1$, that is common knowledge. For this setting, we can still reformulate the problem as a single-parameter mechanism design problem with quasilinear utilities. The difference is that we will consider the translated utility:
\begin{equation}
u_i(b;\val[i]) = \val[i]^{\alpha} \hat{u}_i(r,b_i) = \val[i]^{\alpha} x_i(r(b))-b_i^{\alpha}
\end{equation}
The crucial part in achieving this translation is that the cost of a player depends only on his own bid and is not an expectation over other players values. Thus we can do a completely analogous analysis as in the quasi-linear utility model. The only difference will occur when translating the ability thresholds to badge thresholds, where we would replace $\theta_j$ with 
$\theta_j^{\alpha}$ in all the related Equations \eqref{eqn:effort-to-value} and \eqref{eqn:value-to-effort}.


\vsdelete{\subsection{Asymmetric Ability Distributions}
\subsection{Prior-Free Approximations}
\subsection{Simultaneous Participation in Many Badge Mechanisms}
\section{Discussion}\label{sec:discussion}}


==> general-model.tex <==
% !TEX root=badges.tex



==> large.tex <==
% !TEX root=badges.tex

We show that for a sufficiently large number of players the unique Bayes-Nash equilibrium of a badge mechanism with
a fixed number of badges with quantile thresholds $\tq{1}, \ldots, \tq{m}$ becomes an ex-post
equilibrium. The latter also has implications on the extensive robustness of the Bayes-Nash equilibrium to 
extensive form perturbations of the game, by applying the results of \cite{Kalai2004}.

Our result implies that the single-badge approximate mechanism that we considered in the previous section, results in an approximate ex-post equilibrium for sufficiently large markets and hence  becomes extensively robust. Formally, we 
use the following definition of an approximate ex-post equilibrium and of extensive robustness.
\begin{defn}[\cite{Kalai2004}] A mixed Bayes-Nash equilibrium is $(\epsilon,\rho)$ ex-post Nash if with probability
at least $1-\rho$, no player can improve his utility by more than additively $\epsilon$, after the instantiation of 
the types and strategies.
\end{defn}

Kalai \cite{Kalai2004} shows that if the Bayes-Nash equilibrium becomes an ex-post equilibrium at an exponential rate
in the number of players then this implies that the Bayes-Nash equilibrium is extensively robust, in the following sense.
Consider extensive form versions of the game where players take potentially many turns to play and revise their strategy
and where information about players types can be arbitrarily revealed in between rounds. The sole assumption
required is that for every possible strategy of the simultaneous game, a player has the option in the extensive
form version to play that strategy at the first time he is allowed to play and stick to it for the rest of the game. 
A Bayes-Nash equilibrium of the simultaneous game is extensively robust, if the strategy of playing according
to that equilibrium in the first round you are allowed to play and sticking to the same action for all subsequent
plays, is a Bayes-Nash equilibrium of any extensive form version of the game as described above. It  is $(\epsilon,\rho)$
extensively robust, if with probability $1-\rho$ no player has an $\epsilon$ improving deviation at any information 
set of the extensive form game. Kalai \cite{Kalai2004} shows that if a Bayes-Nash equilibrium becomes an $(\epsilon,\rho)$ ex-post equilibrium, with $\rho$ being exponential in the number of players, then it is also an $(\epsilon,\rho')$ extensively
robust with $\rho'$ also decaying exponentially in the number of players. 

To prove our result we need to adapt the techniques of Kalai \cite{Kalai2004} to our setting. Kalai \cite{Kalai2004}
considers only settings with a finite set of actions and types and with continuous utilities. Our setting involves 
a continuum of types, a continuum of strategies and at a first glance a discontinuous utility. However, due to the monotonicity
of the equilibrium, and the finiteness of the badges, the number of undomianted strategies is finite and 
the number of types is also essentially finite, since all that characterizes a players behavior is whether his type falls in one of finitely many ability intervals. Additionally, we can view the utility of a player as a function of the proportion of players that congest each badge, i.e. the proportion of players that fall within each ability interval. Under such a perspective the utility of a player is a continuous function of this proportions, for any fixed action of the player, due to the continuity 
of the status function. The latter allows us to apply techniques similar to those in \cite{Kalai2004} to show
an exponential convergence to an ex-post Nash equilibrium.

\begin{lemma}\label{lem:large}Consider a badge mechanism with quantile thresholds $\tqvec=(\tq{1}, \ldots, \tq{m})$ and a $c$-Lipschitz status function $\stat{\cdot}$. For any positive $\epsilon$, there exists constants $\alpha$, and $\beta$ that depend on $\epsilon$ and on the instance of the game, such that any Bayes-Nash of the game with $n$ players is $(\epsilon, \alpha \beta^n)$ ex-post equilibrium.
\end{lemma}







==> linear-many.tex <==
%Whilst, the per-user contribution generated by a single badge mechanism is simply $APX= R(\tq{})\cdot (1-\tq{})$, while the revenue
%of an $m$-badge mechanism with quantile thresholds $\tqvec=(\tq{1},\ldots,\tq{m})$ is 
%$$APX=n \cdot \left(R(\tq{1})\cdot(1-\tq{1})+\sum_{t=2}^m R(\tq{t})\left(\tq{t-1}-\tq{t}\right)\right).$$
%A graphical representation of the revenue of the optimal mechanism and that of the $m$-badge mechanism is given in Figure \ref{fig:concave}.
%\begin{figure}[htpb]
%\subfigure{\includegraphics[scale=.8]{optimal-revenue.eps}}
%\subfigure{\includegraphics[scale=.8]{approx-optimal-revenue.eps}}
%\caption{Left figure depicts the per player revenue of the optimal mechanism. The dashed line 
%corresponds to the revenue curve (in this example of the uniform distribution) and the shaded region corresponds to the
%per player optimal revenue. The shaded region in the right figure depicts the per player revenue of a badge mechanism with three quantile thresholds $(\kappa_1,\kappa_2,\kappa_3)$.} \label{fig:concave}
%\end{figure}
%
%Given this graphical interpretation of revenue we show the main result of this section:
%
%
%
%\begin{theorem}\label{thm:linear-m-badge} When the status function is linear then an $m$ badge mechanism can achieve a $\frac{m+2}{m}$
%approximation to the optimal revenue.
%\end{theorem}
%\begin{proof}
%Consider iteratively placing badges at the center of the intervals defined by the previous set of badges and the points $0$
%and $1$. After adding such a set of badges, by the same reasoning as in Lemma \ref{lem:linear}, the remnant of 
%the optimal revenue that is not accounted for in the badge mechanism is reduced by half. Thus after $t$ such iterations
%we get that the resulting badge mechanism gets a $1-\frac{1}{2^t}$ fraction of the optimal. Observe that if
%at step $t$ we had $m_t$ badges, then at step $t+1$ we have $2m_t+1$ badges. Since $m_1=1$, we get
% that at step $t$ we have $2^{t}-1$ badges. Thus if we use $m\in [2^{t}-1,2^{t+1}-1)$ badges we can achieve
%$1-\frac{1}{2^t}\geq 1-\frac{2}{m+2}$ fraction of the optimal.
%\end{proof}
%Observe that the approximately optimal badges used in the proof of Theorem \ref{thm:linear-m-badge} divide the 
%quantile space above the monopoly quantile in equal intervals. This implies that for the case of linear status, a practical rule of thumb for the designer is to set his badges so that the expected number of players in each non-zero status class is the same.
%
%
%We also generalize the theorem above to show how the badge mechanism revenue converges to the optimal revenue, as 
%the number of badges $m$ used increases.

\begin{theorem}\label{thm:many-badge-concave}
If the social status function $\stat{\cdot}$ is concave, then a badge mechanism with $m$ badges, can achieve a $\frac{m}{m-2}$-approximation to the optimal revenue. 
\end{theorem}
\vscomment{The proof in the appendix uses very old notation. Fix this!}


==> linear-many.tex.old.tex <==
Whilst, the per-user contribution generated by a single badge mechanism is simply $APX= R(\tq{})\cdot (1-\tq{})$, while the revenue
of an $m$-badge mechanism with quantile thresholds $\tqvec=(\tq{1},\ldots,\tq{m})$ is 
$$APX=n \cdot \left(R(\tq{1})\cdot(1-\tq{1})+\sum_{t=2}^m R(\tq{t})\left(\tq{t-1}-\tq{t}\right)\right).$$
A graphical representation of the revenue of the optimal mechanism and that of the $m$-badge mechanism is given in Figure \ref{fig:concave}.
\begin{figure}[htpb]
\subfigure{\includegraphics[scale=.8]{optimal-revenue.eps}}
\subfigure{\includegraphics[scale=.8]{approx-optimal-revenue.eps}}
\caption{Left figure depicts the per player revenue of the optimal mechanism. The dashed line 
corresponds to the revenue curve (in this example of the uniform distribution) and the shaded region corresponds to the
per player optimal revenue. The shaded region in the right figure depicts the per player revenue of a badge mechanism with three quantile thresholds $(\kappa_1,\kappa_2,\kappa_3)$.} \label{fig:concave}
\end{figure}

Given this graphical interpretation of revenue we show the main result of this section:



\begin{theorem}\label{thm:linear-m-badge} When the status function is linear then an $m$ badge mechanism can achieve a $\frac{m+2}{m}$
approximation to the optimal revenue.
\end{theorem}
\begin{proof}
Consider iteratively placing badges at the center of the intervals defined by the previous set of badges and the points $0$
and $1$. After adding such a set of badges, by the same reasoning as in Lemma \ref{lem:linear}, the remnant of 
the optimal revenue that is not accounted for in the badge mechanism is reduced by half. Thus after $t$ such iterations
we get that the resulting badge mechanism gets a $1-\frac{1}{2^t}$ fraction of the optimal. Observe that if
at step $t$ we had $m_t$ badges, then at step $t+1$ we have $2m_t+1$ badges. Since $m_1=1$, we get
 that at step $t$ we have $2^{t}-1$ badges. Thus if we use $m\in [2^{t}-1,2^{t+1}-1)$ badges we can achieve
$1-\frac{1}{2^t}\geq 1-\frac{2}{m+2}$ fraction of the optimal.
\end{proof}
Observe that the approximately optimal badges used in the proof of Theorem \ref{thm:linear-m-badge} divide the 
quantile space above the monopoly quantile in equal intervals. This implies that for the case of linear status, a practical rule of thumb for the designer is to set his badges so that the expected number of players in each non-zero status class is the same.


We also generalize the theorem above to show how the badge mechanism revenue converges to the optimal revenue, as 
the number of badges $m$ used increases.

\begin{theorem}\label{thm:many-badge-concave}
If the social status function $\stat{\cdot}$ is concave, then a badge mechanism with $m$ badges, can achieve a $\frac{m}{m-2}$-approximation to the optimal revenue. 
\end{theorem}
\vscomment{The proof in the appendix uses very old notation. Fix this!}


==> linear.tex <==
% !TEX root=badges.tex






==> optimal-badge.tex <==
% !TEX root=badges.tex

%Before analyzing how badges compare to the optimal hypothetical mechanism, we first turn to the question of computing 
%the optimal badge mechanism, subject to the restriction of using only $m$ badges. We give an algorithmic result, showing that
%there exists a fully polynomial time approximation scheme that computes the optimal badge thresholds.
%
%Using our equilibrium characterization we can compute the expected revenue produced by a set of badges with thresholds $\kappa=(\kappa_1,\ldots,\kappa_m)$ in the quantile space as follows: For notational convenience assume that $\kappa_0=1$
%with $\hat{x}(\kappa_0)=0$ and $\kappa_{m+1}=0$ with $\hat{x}(\kappa_{m+1})=1$. If a player has quantile $q_i\in [\kappa_j,\kappa_{j+1}]$ then by transforming Equation
%\eqref{eqn:effort-to-value} we get that he submits a bid of $\theta_j= \sum_{t=1}^j v(\kappa_t)\left(\hat{x}(\kappa_t)-\hat{x}(\kappa_{t-1})\right)$. The latter happens with probability $\kappa_j - \kappa_{j+1}$. Thus a player's expected payment is:
%\begin{align*}
%\E_{v_i}[b(v_i)] =~&\sum_{j=1}^m\sum_{t=1}^j (\kappa_j-\kappa_{j+1}) v(\kappa_t)\left(\hat{x}(\kappa_t)-\hat{x}(\kappa_{t-1})\right)\\
%=~& \sum_{t=1}^m \sum_{j=t}^m  (\kappa_j-\kappa_{j+1}) v(\kappa_t)\left(\hat{x}(\kappa_t)-\hat{x}(\kappa_{t-1})\right)\\
%=~& \sum_{t=1}^m  \left(v(\kappa_t)\left(\hat{x}(\kappa_t)-\hat{x}(\kappa_{t-1})\right) \sum_{j=t}^m  (\kappa_j-\kappa_{j+1})\right)\\
%=~& \sum_{t=1}^m  v(\kappa_t)\left(\hat{x}(\kappa_t)-\hat{x}(\kappa_{t-1})\right)(\kappa_t - \kappa_{m+1})\\
%=~& \sum_{t=1}^m \kappa_t \cdot v(\kappa_t)\cdot \left(\hat{x}(\kappa_t)-\hat{x}(\kappa_{t-1})\right)\\
%=~& \sum_{t=1}^m R(\kappa_t)\cdot \left(\hat{x}(\kappa_t)-\hat{x}(\kappa_{t-1})\right)
%\end{align*}
%Since players are drawn from the same distribution the expected total revenue of the badge mechanism is simply $n$ times the 
%expected revenue contribution of each individual player. Observe that the contribution of a badge $t$ to the revenue depends only on the values of $\kappa_t$ and $\kappa_{t-1}$. Specifically, if we denote with
%\begin{equation}
%T(q,q') = R(q)\cdot\left(\hat{x}(q)-\hat{x}(q')\right)
%\end{equation}
%Then the revenue of a badge mechanism with $m$ thresholds can be written as:
%\begin{equation*}
%\E_{v}\left[\sum_i b(v_i)\right] = n\sum_{t=1}^m T(\kappa_t,\kappa_{t-1})
%\end{equation*}
%The latter implies a dynamic programming approach for computing the optimal quantile thresholds (which would then yield the optimal
%badge thresholds). Let $C(x,m)$ denote the optimal revenue achievable with $m$ badges subject to the constraint that the last badge has quantile threshold $x$. Then we obtain the recursive equation:
%\begin{equation}
%C(x,m) = \max_{y\in [x,1]}\left\{ T(x,y)+C(y,m-1) \right\}
%\end{equation}
%with $C(x,1)$ simply being the revenue of the badge mechanism with a single quantile threshold of $x$. If the quantiles were discrete, taking values among a set of $T$ finite values, then the latter would imply a dynamic programming 
%algorithm that runs in time $O(T^2\cdot m)$.
%Hence, we can discretize the quantile space in multiples of $\delta$, which would yield some error $\epsilon$ that is polynomial in $\delta$ and would require $O(m/\delta^2)$ time to run.

%\begin{example}(Optimal Single Badge) To give a qualitative insight of an optimal badge, we give
%here an example of what is the optimal single badge. The revenue of a single badge with quantile threshold $x$ yields revenue of $v(x)\left(1-(1-x)^n\right)$ or equivalently the revenue of a badge with ability thresholds $a$ yields revenue: $a(1-F(a)^n)$. The latter is exactly the revenue of a single item auction with one buyer drawn from the distribution $F^n$ of the maximum ability among $n$ players. Thus the optimal ability threshold is to set a badge that corresponds to the monopoly reserve of this distribution: i.e. the solution to the equation $a=\frac{1-F(a)^n}{n\cdot f(a)\cdot F(a)^{n-1}}$. To implement such an ability threshold the designer needs to set the badge threshold to satisfy the equation: 
%$$\theta=a\cdot \tilde{x}(a) = a \cdot \frac{1-F(a)^n}{n\cdot(1-F(a))} $$
%For instance if the abilities where drawn uniformly in $[0,1]$, then the optimal ability threshold would be: $a=(n+1)^{-1/n}$ and the corresponding optimal badge threshold would be: $\theta=\frac{1}{(n+1)\cdot\left((n+1)^{1/n}-1\right)}$.
%\end{example}


%\vscomment{Started fixing this section.} \subsection{Comparison with Optimal Ranking Mechanism with Restricted Ranks} We have seen that with logarithmic number of badges we can approximate to within a constant factor any possible ranking mechanism. However, how does the optimal badge mechanism with $m$ badges compare to the optimal ranking mechanism with the analogous handicap of being able to use only $m$ ranks?
%
%\textbf{Optimal Ranking Mechanism with $m$ Ranks.} We first analyze what is the optimal ranking mechanism restricted to $m$ ranks. By arguments similar to Section \ref{sec:optimal} we know that the optimal ranking mechanism is the one that maximizes the virtual welfare. However, when
%we restricted the amount of ranks that the mechanism can use, Lemma \ref{lem:optimal-welfare} is no longer true and the optimal virtual welfare
%mechanism doesn't have a clean structure. Specifically, it is not optimal for instance, for the top $m-1$ players to receive a distinct rank and for 
%the remaining players that pass the monopoly reserve to be awarded the last rank, rather it might be better to group people together in ranks as 
%the following example shows.
%
%\begin{example} Consider an instance with $n=7$ players with equal ability of $v_i=1$ and $m=4$ ranks. Then having $1$ player in each of the 
%top $2$ ranks, $2$ players in the third rank and $3$ players in the last rank, achieves higher welfare than having $1$ player in each of the top $3$ 
%ranks and $4$ players in the last rank. 
%\end{example}
%
%Hence, in general the optimal partition of the players will be a complex function of their virtual values. However, we show that the optimal mechanism
%always awards the top rank only to one person. 
%\begin{lemma} In the optimal mechanism, only one person is awarded the highest rank.\end{lemma}
%
%Hence, at least for the case of two ranks we know that the optimal ranking mechanism awards the first rank to the highest ability player and awards the second rank to every player that passes the monopoly reserve. 

%
%It is easy to see that if we are restricted to assigning $m$ ranks, then the optimal achievable welfare is to order players in decreasing order of
%value and assign decreasing distinct ranks to the top $m-1$ players, while assigning the $m$-th rank to all the remaining players. Thus for regular i.i.d. settings the virtual welfare maximizing mechanism is the one that assigns rank $0$ to all
%players that have negative virtual value (i.e. don't pass the monopoly reserve of $F$) and then do the welfare maximizing 
%allocation for the remaining players, as described above. Last, as usual the optimal mechanism asks the players to submit an output that follows the payment identity corresponding to the interim allocation rule implied by the above ex-post allocation rule.
%
%For the case of a single badge, comparing the optimal badge mechanism to the optimal restricted rank mechanism, essentially boils down to comparing the optimal posted price mechanism (i.e. post a price and award uniformly at random to anyone who passes it) with the optimal single-item auction for i.i.d. regular environments. The two auctions are known by Chawla et al \cite{Chawla} to be within a factor of $2$ of each other. Hence, our theorem corresponds to a generalization of this theorem for many badges, showing that for any $m$ badges the optimal badge mechanism is a $2$ approximation to the optimal ranking mechanism restricted to $m$ ranks.



Given the above characterization of revenue in a badge mechanism, a natural question is whether an extra badge can actually hurt revenue. We
show that this cannot happen as long as the quantile threshold of this extra badge is above the monopoly quantile of the distribution. 

\begin{lemma}Adding an extra badge with quantile threshold $\tilde{\kappa}\geq \kappa^*$ can only increase the revenue of an existing
badge mechanism. 
\end{lemma}
\begin{proof}
%The revenue of badge mechanism with quantile thresholds $\kappa=(\kappa_1,\ldots,\kappa_m)$ can be rewritten as:
%\begin{equation}
%REV_{\kappa}=\sum_{t=1}^{m}(R(\kappa_t)-R(\kappa_{t+1}))\cdot \hat{x}(\kappa_t)
%\end{equation}
%where we assumed that $\kappa_{m+1}=0$ and hence $R(\kappa_{m+1})=0$.
Consider augmenting the badge mechanism with an extra badge with quantile threshold $\tilde{\kappa}$ and such that $\tilde{\kappa}\in [\kappa_{t+1},\kappa_t]$ for some $t\in [1,m]$, with the convention that $\kappa_{m+1}=0$ and $\kappa_{0}=1$. Then the revenue of this new mechanism is:
\begin{equation*}
REV_{\kappa+\tilde{\kappa}}=\sum_{\sigma \neq t }(R(\kappa_t)-R(\kappa_{t+1})\cdot \hat{x}(\kappa_t) +(R(\kappa_t)-R(\tilde{\kappa}))\cdot \hat{x}(\kappa_t)+
(R(\tilde{\kappa})-R(\kappa_{t+1}))\cdot \hat{x}(\tilde{\kappa})
\end{equation*}
By regularity of the distribution, we know that $R(\cdot)$ is monotone in the region $[0,\kappa^*]$. Since we assumed that $\tilde{\kappa}\leq \kappa^*$
we get that $R(\tilde{\kappa})\geq R(\kappa_{t+1})$. By monotonicity of $\hat{x}(\cdot)$ we also have: $\hat{x}(\tilde{\kappa})\geq \hat{x}(\kappa_t)$. 
Combining the above we get the Lemma:
\begin{align*}
REV_{\kappa+\tilde{\kappa}}\geq~& \sum_{\sigma \neq t }(R(\kappa_t)-R(\kappa_{t+1})\cdot \hat{x}(\kappa_t) +(R(\kappa_t)-R(\tilde{\kappa}))\cdot \hat{x}(\kappa_t)+
(R(\tilde{\kappa})-R(\kappa_{t+1}))\cdot \hat{x}(\kappa_t)\\
=~&\sum_{\sigma \neq t }(R(\kappa_t)-R(\kappa_{t+1})\cdot \hat{x}(\kappa_t) +(R(\kappa_t)-R(\kappa_{t+1}))\cdot \hat{x}(\kappa_t)=REV_{\kappa}
\end{align*}
\end{proof}












==> optimal-nsi.tex <==
% !TEX root=badges.tex

{\bf NSI: surplus vs welfare vs ability?}

We will use the framework of optimal auction design to design the optimal badge mechanism.  To this end, it is useful to work in quantile space and scale the utility functions of the players by their values.  After doing so, the utility function of a player becomes:
\begin{equation}
u_i(\bvec;\quant[i]) = \val(\quant[i]) \cdot \stat{t_i} - b_i.
\end{equation}
Comparing with equation~(\ref{eqn:standardutil}), we see the status of a player equates with the allocation of an agent in the auction literature and the payment equates with contribution.  The badge mechanism that maximizes contributions is thus functionally equivalent to the optimal (revenue-maximizing) auction.  Note our setting exhibits two key restrictions not present in standard optimal auction design:
\begin{enumerate}
\item The set of feasible allocations (status values) is highly constrained and ill-behaved due to the externalities that a player's status imposes on others.  In particular, the total amount of allocation, i.e., $\sum_i\stat{t_i}$ is not constant as in the standard auction setting discussed in Section~\ref{sec:preliminaries}.
\item The payments (contributions) are not determined by the mechanism, but rather by the players themselves.  In this sense, a badge mechanism is a special type of auction, known in the literature as an all-pay auction.
\end{enumerate}

The optimal auction framework states that the optimal mechanism chooses an interim allocation rule which maximizes expected virtual surplus and then computes payments which support these interim allocations in equilibrium (see Section~\ref{sec:preliminaries}).  Following this reasoning, we first compute the surplus-maximizing allocation.  We then argue this allocation is implemented in a BNE by a {\em leaderboard with a contribution cutoff}.  Finally, we show that the derived BNE is unique.

\subsection{Surplus-Maximizing Allocation}

Maximizing virtual surplus for some instantiation of a quantile profile $\qvec$ is simply an optimization problem, subject to the
constraints that are implicit in the way that players derive status. The optimization problem asks: given a vector of virtual abilities $R'(\quant[1]),\ldots,R'(\quant[n])$, assign badges $\rvec=(\rank_1,\ldots,\rank_n)$ to the players so as to maximize: $\sum_i R'(\quant[i])\cdot \stat{t_i(\rvec)}$. The following lemma states that the solution assings players distinct badges in decreasing order of their quantile so long as their quantile is below the {\em monopoly quantile} $\tqstar{}$ (equivalently, so long as their virtual ability is non-negative), and assigns all other players a badge of $0$. The formal proof is deferred to the appendix.

\begin{lemma}[Virtual Welfare Maximizing Badge Allocation]\label{lem:optimal-welfare} 
Let $\quant[1]\leq \ldots \leq \quant[k]\leq \tqstar< \quant[k+1]\leq \ldots \leq \quant[n]$ be a profile of quantiles. Then the optimal virtual welfare is achieved by assigning a distinct decreasing badge to all players $\{1,\ldots,k\}$ with non-negative virtual ability and badge $0$, to all negative virtual ability players $\{k+1,\ldots,n\}$, i.e. $r_1=n, r_2=n-1,\ldots, r_k=n-k+1$, and $r_{k+1}=\ldots=r_n=0$. Such an allocation of badges produces virtual welfare of:
\begin{equation*}
\sum_{i=1}^{n}R'(\quant[i])\cdot \stat{t_i} =\sum_{i=1}^{k} R'(\quant[i])\cdot \stat{\frac{i-1}{n-1}}.
\end{equation*} 
\end{lemma}

\subsection{Implementation}

We now show that the ex-post virtual welfare maximizing allocation of badges is implemented at an equilibrium of a \emph{leaderboard with a contribution cutoff}: players are assigned a badge in decreasing order of contribution (breaking ties at random) as long as they pass an appropriately chosen contribution threshold of $\theta$.  To do so, we need to show two things: first, we must describe the interim allocation rule implied by the ex-post allocation rule in Lemma~\ref{lem:optimal-welfare}.  Then we must compute corresponding bids using the payment identity of the optimal auction framework and check that these bids do indeed give rise to the interim allocation.

To compute the interim allocation, let $T_i$ be the random variable denoting the number of opponents with quantile smaller than $\quant[i]$. Then the implied interim allocation of a player with $\quant[i]\leq \tqstar$ is $\E_{\qvec_{-i}}\left[S\left(\frac{T_i}{n-1}\right)\right]$ and with $\quant[i]>\tqstar$ is simply $0$. Since $T_i$ is distributed as a Bernoulli distribution of $n-1$ independent random trials, each with success probability of $\quant[i]$,\footnote{Recall that quantiles are distributed uniformly in $[0,1]$.} we can write the interim status allocation of a player with quantile $\quant[i]\leq \tqstar$ as:
\begin{equation}\label{eqn:badge-interim}
\xq{\quant[i]}=  \sum_{\nu=0}^{n-1}\stat{\frac{\nu}{n-1}}\cdot \beta_{\nu,n-1}(\quant[i])
\end{equation}
where $\beta_{\nu,n}(q)= \binom{n-1}{\nu}\cdot q^{\nu}\cdot (1-q)^{n-1-\nu}$, denotes the Bernstein basis polynomial and $\xq{\quant}$ is the Bernstein polynomial approximation of the status function $\stat{\cdot}$. By properties of Bernstein polynomials (see \cite{phillips-bernstein}), if $\stat{\cdot}$ is a strictly decreasing function then $\xq{\cdot}$ is also strictly decreasing and if $\stat{\cdot}$ is convex or concave then so is $\xq{\cdot}$. Additionally, $\xq{\cdot}$ is continuous and differentiable and $\xq{0}=\stat{0}$ and $\xq{1}=\stat{1}=0$. 

We now derive the bids using the payment identity.

\begin{theorem}[Optimal Badge Mechanism: Leaderboard with a cutoff]\label{thm:optimal}
The optimal badge mechanism assigns a distinct badge to each all players in decreasing order of contribution (breaking ties at random) as long as they pass a contribution threshold of $\theta=\val(\tqstar)\cdot\xq{\tqstar}$. Player's that don't pass the contribution threshold are assigned a badge of $0$.
\end{theorem}
\begin{proof}
The proof consists of two parts: First we show that the interim allocation of status $\xq{\quant}=\statn{n}{\quant}\cdot {\bf 1}_{\quant\leq \tqstar}$ given above, together with the contribution function given in Lemma \ref{lem:myerson}, constitute an equilibrium of the badge mechanism. To achieve this we simply need to verify that the implied contribution function, indeed gives rise to the optimal interim allocation of status. Then by Lemma \ref{lem:myerson} and after also checking that players don't want to bid outside of the region of contrbituions spanned by $b(\cdot)$, this pair of $\xq{\cdot}$ and $b(\cdot)$ are an equilibrium. Second, we need to argue that the mechanism has no other equilibria. To achieve this, we show that this specific form of a badge mechanism, falls into the class of anonymous order-based auctions of Chawla and Hartline \cite{Hartline2012}, where it is shown that such auctions have unique equilibria.

The contribution function implied by Lemma \ref{lem:myerson}, when instantiated for interim status allocation of $\statn{n}{\quant}{\bf 1}_{\quant\leq \tqstar}$ gives, that each player's equilibrium contribution as a function of his quantile must satisfy:
\begin{equation*}
b(\quant) = \begin{cases}
\val(\quant)\cdot \statn{n}{\quant}+\int_{\quant}^{\tqstar}\statn{n}{z}\cdot \val'(z)\cdot dz & \text{if $\quant\leq \tqstar$}\\
0 & \text{o.w.}
\end{cases}
\end{equation*}
Observe that the above bid function is a strictly decreasing in the region $[0,\tqstar]$, since $b'(\quant)=\val(\quant)\cdot \statnpr{n}{\quant}$, and both $\val(\cdot)$ and $\statn{n}{\cdot}$ are strictly decreasing functions. Moreover, 
observe that $b(\tqstar)=\val(\tqstar)\cdot \statn{n}{\tqstar}=\theta$. Since all quantiles are distributed uniformly in $[0,1]$, under the above bid function, a player with quantile $\quant\leq \tqstar$ is assigned a badge lower than every player with higher quantile and higher than every player with lower quantile, while the event of a tie has zero measure. Thereby, the latter
bid function $b(\cdot)$, gives rise to the optimal interim allocation of status $\statn{n}{\quant}\cdot {\bf 1}_{\quant\leq \tqstar}$. Last, it is easy to see that since the player with quantile $0$, doesn't want to bid above $b(0)$ (since he gets the same status at a higher cost), no player wants to bid above the bid $b(0)$. That latter follows from the fact that the characterization in Lemma \ref{lem:myerson} guarantees that no player wants to deviate to any bid in the region of bids spanned by $b(\cdot)$ and hence $b(0)$. From this it immediately follows that they also don't want to bid above $b(0)$. Additionally, it is also trivial to see that no player wants to bid in the region $(0,\theta)$. Thus we can conclude that the above pair of interim allocation and contribution function are an equilibrium of the mechanism.
\end{proof}

\subsection{Uniqueness}

The fact that the badge mechanism has a unique equilibrium, follows from the recent results of Chawla and Hartline \cite{Hartline2012}. Despite the fact that general badge mechanisms do not fall into the class of auctions studied in \cite{Hartline2012} (such as for instance absolute threshold badge mechanisms), the specific leaderboard with a cutoff badge
mechanism fall into their framework. To show this, we need to argue that for any contribution profile $\bvec$ (even in the case of tied contributions), the ex-post expected allocation of status of a player depends only on his own contribution, on the number of players that have a higher contribution and on the number of players that have the same contribution (but for instance, not on the exact contributions of other players). Since, ties are broken uniformly at random, a player is ranked above another player with an equal contribution with probability of $1/2$. Thus if we denote with $n_g(\bvec)$ the number of players that contribute more and with $n_e(\bvec)$ the number of players with an equal contribution, then the expected ex-post status allocation of a player is:
\begin{equation*}
\sum_{\nu=0}^{n_e(\bvec)}\stat{\frac{n_g(\bvec)+n_e(\bvec)}{n-1}}\cdot \beta_{\nu,n_e(\bvec)}(1/2)
\end{equation*}
when his contribution $b_i\geq \theta$ and $0$ otherwise. It is clear that this ex-post allocation only depends on the quantities required by the framework of \cite{Hartline2012}.

Observe that the optimal badge mechanism described above has two main drawbacks. First the equilibrium contribution is a very complex function of the ability distribution, and therefore, small errors in a player's beliefs will dramatically change the total contribution that would arise in practice. Second, the optimal mechanism is not detail-free, as it depends on the monopoly quantile of the distribution. In the sections that follow we will address each of these issues separately and we will give approximately optimal badge mechanisms that avoid some of these drawbacks. 

Specifically, we will show that a very simple badge mechanism that is defined via an absolute contribution threshold, in a way that at equilibrium, half of the population acquires the top badge, is a $4$-approximation to the optimal badge mechanism when the status function is concave. For the players to decide how to play in this simple single absolute threshold mechanism it suffices to have correct beliefs only about the median ability, which seems a much smaller cognitive burden. We also address how a good approximation can be achieved by a multi-level absolute contribution threshold badge mechanism, with a small number of thresholds and even for convex status functions. Moreover, when the status function is convex, we show that the detail-free mechanism, that simply ranks the players in decreasing order of contribution (i.e. a leaderboard) achieves a $2$-approximation to the optimal total contribution.



==> optimal.tex.old.tex <==
% !TEX root=badges.tex

%Intuitively, a badge mechanism induces a ranking among players; the players who win the highest badge are assigned the highest status class, players who win the second highest badge are assigned the second highest status class, and so on. These badge-induced rankings are just one example of a general mechanism which collects contributions from agents and assigns status class based on that output. For example, we could collect contributions and then assign the highest contributor to the highest status class, the second highest contributor to the next status class, etc. Another mechanism could assign the 10 highest contributors to the highest status class, then the next 100 highest contributors to the second highest status class, and the lowest status class to every other player.
%
%Along the same lines, one could ask the question of how does a badge mechanism with a fixed or small number of badges compare with respect to a mechanism with
%a continuum of badges (observe that giving the designer the freedom to add more badges can only increase optimal revenue). A continuum of badges 
%can simulate any symmetric ranking mechanism where status class is monotone in ability. For instance, it can simulate the mechanism where every player is assigned a distinct status class.

%In this section, we show that the optimal mechanism  is a fully discriminatory one which assigns a distinct status class to each player in decreasing order of submitted contributions, subject to each contribution being above a certain threshold. Any player that submits a contribution below the threshold is assigned a status class of 0. In the next section we show that a simple badge mechanism provides a good approximation to the optimal mechanism. 
%
%We first introduce the optimal mechanism design problem. Suppose the designer is allowed to run an arbitrary mechanism that asks each player to report his quantile, and then outputs a status class profile $r=(r_1,\ldots,r_n)$ and an output profile $b=(b_1,\ldots,b_n)$, such that each player $i$ contributes $b_i$ and is assigned status class $r_i$. Each player's utility for any such output is of the form $u_i(r,b_i) = \val(\quant[i])\cdot x_i(r) - b_i$, where $x_i(r)$ is as defined in the Section \ref{sec:model}. The only restriction we make on the mechanism is that each player's expected utility is non-negative, i.e. it is rational for participate in the mechanism. What is the mechanism that produces the highest expected revenue in Bayes-Nash equilibrium?
%
%This scenario is the classic single-parameter optimal mechanism design setting with quasi-linear utilities. By the Revelation Principle the designer can restrict himself to direct Bayesian incentive compatible mechanisms of the form: players report their abilities, the designer decides an allocation of status classes based on the reported abilities, and then asks the players to output some $b_i$ such that truthfully reporting ability is an equilibrium for all players in the resulting game of incomplete information. 

%Before computing the revenue-optimal allocation, we compute the welfare-optimal allocation. The social welfare in this setting is defined as the sum of all agents utilities plus the utility for the designer. The utility for the designer is equal to the sum of the output for the agents. For a given vector of abilities $v$, an allocation of status classes $r$ and a vector of agent outputs $b$, the social welfare is as follows. 
%\begin{equation}
%SW(\quant,r,b) = SW_{players}  + SW_{designer} = \sum_i \val(\quant[i]) \cdot x_i(r) 
%\end{equation}
%
%In words, each agent's contribution to the social welfare is equal to his ability weighted by status value. The following lemma shows welfare is maximized\footnote{This lemma is not characterizing the welfare-optimal because we transformed utilities in equation 4. However, this lemma is useful for characterizing the revenue-optimal mechanism.} by assigning assigning each player a different status class in decreasing order of ability. 
%
%\begin{lemma}\label{lem:optimal-welfare} 
%If $\quant[1]\leq \quant[2]\leq \ldots \leq \quant[n]$ then the optimal social welfare is achieved by assigning $r_1=n, r_2=n-1,\ldots, r_n=1$, producing welfare of:
%\begin{equation*}
%\sum_i\val(\quant[i])\cdot x(r) =\sum_i \val(\quant[i])\cdot \stat{\frac{i-1}{n-1}}
%\end{equation*} 
%\end{lemma}
%\begin{proof}
%The statement follows by the following arguments: first it is easy to see that the status class should be monotone non-decreasing in the value, since if 
%$\val(\quant[i])>\val(\quant[j])$ and $r_i<r_j$ then we can increase welfare by swapping the status class of player $i$ and player $j$. Additionally, if for some set of values 
%$\val(\quant[i])\geq \val(\quant[i+1])\geq \ldots \val(\quant[i+k])$ we have $r_i=\ldots = r_{i+k}$ then by discriminating $\val[i]$ to be strictly higher than the rest of the values
%increases the welfare. More concretely, for any $j> i$ we can set $r_j'=r_j+1$. The satisfaction of all players $j>i$ doesn't change since the number
%of people that have status class at least as high as them remains the same. Additionally, the satisfaction of player $i$ strictly increases, since the number of 
%people ranked at least as high as him, strictly decreased. 
%\end{proof}

%% NSI: clean up below paragraph; also welfare vs ability?

Lemma \ref{lem:myerson} implies that if the equilibrium of a mechanism maximizes virtual welfare ex-post, then it
achieves a total contribution at least as much as that achieved by any mechanism and is thereby optimal. Therefore, a
first step in characterizing the optimal badge mechanism is to characterize the virtual welfare maximizing allocation of badges for each instantiation of player virtual abilities. We then show how such an allocation can be implemented by a \emph{leaderboard with a contribution cutoff}.  We further show that this mechanism has a unique equilibrium.

Maximizing virtual welfare for some instantiation of a quantile profile $\qvec$, is simply an optimization problem, subject to the
constraints that are implicit in the way that players derive status. The optimization problem asks: given a vector of virtual abilities $R'(\quant[1]),\ldots,R'(\quant[n])$, assign badges $\rvec=(\rank_1,\ldots,\rank_n)$ to the players so as to maximize: $\sum_i R'(\quant[i])\cdot \stat{t_i(\rvec)}$. By simple arguments we can show the following Lemma, whose formal proof is deferred to the appendix.

\begin{lemma}[Virtual Welfare Maximizing Badge Allocation]\label{lem:optimal-welfare} 
Let $\quant[1]\leq \ldots \leq \quant[k]\leq \tqstar< \quant[k+1]\leq \ldots \leq \quant[n]$ be a profile of quantiles. Then the optimal virtual welfare is achieved by assigning a distinct decreasing badge to all players $\{1,\ldots,k\}$ with non-negative virtual ability and badge $0$, to all negative virtual ability players $\{k+1,\ldots,n\}$, i.e. $r_1=n, r_2=n-1,\ldots, r_k=n-k+1$, and $r_{k+1}=\ldots=r_n=0$. Such an allocation of badges produces virtual welfare of:
\begin{equation*}
\sum_{i=1}^{n}R'(\quant[i])\cdot \stat{t_i(\rvec)} =\sum_{i=1}^{k} R'(\quant[i])\cdot \stat{\frac{i-1}{n-1}}
\end{equation*} 
\end{lemma}

Lemma \ref{lem:optimal-welfare} and Lemma \ref{lem:myerson}, imply that optimal total contribution is achieved if, at equilibrium, players are assigned a distinct badge in decreasing order of their quantile, so long as their quantile is below the \emph{monopoly quantile} $\tqstar{}$ or equivalently so long as their virtual ability is non-negative. Players, with negative virtual ability should be assigned the lowest badge $0$. 

Observe that if this is the case, and if we let $T(\quant[i])$ be the random variable denoting the number of opponents with quantile smaller than $\quant[i]$, then the implied interim allocation of status of a player with $\quant[i]\leq \tqstar$ is $\E_{\qvec_{-i}}\left[S\left(\frac{T(\quant[i])}{n-1}\right)\right]$ and with $\quant[i]>\tqstar$ is simply $0$. Since $T(\quant[i])$ is distributed as a Bernoulli distribution of $n-1$ independent random trials, each with success probability of $\quant[i]$,\footnote{We remind that quantiles are distributed uniformly in $[0,1]$} we can write the interim status allocation of a player with quantile $\quant\leq \tqstar$ as:
\begin{equation}\label{eqn:badge-interim}
\xq{\quant[i]} = \statn{n}{\quant[i]} =  \sum_{\nu=0}^{n-1}\stat{\frac{\nu}{n-1}}\cdot \beta_{\nu,n-1}(\quant[i])
\end{equation}
where $\beta_{\nu,n}(x)= \binom{n-1}{\nu}\cdot x^{\nu}\cdot (1-x)^{n-1-\nu}$, denotes the Bernstein basis polynomial and $\statn{n}{x}$ is the Bernstein polynomial approximation of the status function $\stat{x}$. By properties of Bernstein polynomials (see \cite{phillips-bernstein}), if $\stat{x}$ is a strictly decreasing function then $\statn{n}{x}$ is also strictly decreasing and if $\stat{x}$ is convex or concave then so is $\statn{n}{x}$. Additionally, $\statn{n}{x}$ is continuous and differentiable and $\statn{n}{0}=\stat{0}$ and $\statn{n}{1}=\stat{1}=0$. 

We show that the ex-post virtual welfare maximizing allocation of badges is implemented at the unique equilibrium of a badge mechanism that takes the form of a \emph{leaderboard with an absolute cutoff}: players are assigned a badge in decreasing order of contribution (breaking ties at random) as long as they pass an appropriately chosen, absolute contribution threshold of $\theta$. Therefore, by all the preceding reasoning such a mechanism is optimal among all badge mechanisms.

\begin{theorem}[Optimal Badge Mechanism: Leaderboard with a cutoff]\label{thm:optimal}
The optimal badge mechanism assigns a distinct badge to each all players in decreasing order of contribution (breaking ties at random) as long as they pass a contribution threshold of $\theta=\val(\tqstar)\cdot\statn{n}{\tqstar}$. Player's that don't pass the contribution threshold are assigned a badge of $0$.
\end{theorem}
\begin{proof}
The proof consists of two parts: First we show that the interim allocation of status $\xq{\quant}=\statn{n}{\quant}\cdot {\bf 1}_{\quant\leq \tqstar}$ given above, together with the contribution function given in Lemma \ref{lem:myerson}, constitute an equilibrium of the badge mechanism. To achieve this we simply need to verify that the implied contribution function, indeed gives rise to the optimal interim allocation of status. Then by Lemma \ref{lem:myerson} and after also checking that players don't want to bid outside of the region of contrbituions spanned by $b(\cdot)$, this pair of $\xq{\cdot}$ and $b(\cdot)$ are an equilibrium. Second, we need to argue that the mechanism has no other equilibria. To achieve this, we show that this specific form of a badge mechanism, falls into the class of anonymous order-based auctions of Chawla and Hartline \cite{Hartline2012}, where it is shown that such auctions have unique equilibria.

The contribution function implied by Lemma \ref{lem:myerson}, when instantiated for interim status allocation of $\statn{n}{\quant}{\bf 1}_{\quant\leq \tqstar}$ gives, that each player's equilibrium contribution as a function of his quantile must satisfy:
\begin{equation*}
b(\quant) = \begin{cases}
\val(\quant)\cdot \statn{n}{\quant}+\int_{\quant}^{\tqstar}\statn{n}{z}\cdot \val'(z)\cdot dz & \text{if $\quant\leq \tqstar$}\\
0 & \text{o.w.}
\end{cases}
\end{equation*}
Observe that the above bid function is a strictly decreasing in the region $[0,\tqstar]$, since $b'(\quant)=\val(\quant)\cdot \statnpr{n}{\quant}$, and both $\val(\cdot)$ and $\statn{n}{\cdot}$ are strictly decreasing functions. Moreover, 
observe that $b(\tqstar)=\val(\tqstar)\cdot \statn{n}{\tqstar}=\theta$. Since all quantiles are distributed uniformly in $[0,1]$, under the above bid function, a player with quantile $\quant\leq \tqstar$ is assigned a badge lower than every player with higher quantile and higher than every player with lower quantile, while the event of a tie has zero measure. Thereby, the latter
bid function $b(\cdot)$, gives rise to the optimal interim allocation of status $\statn{n}{\quant}\cdot {\bf 1}_{\quant\leq \tqstar}$. Last, it is easy to see that since the player with quantile $0$, doesn't want to bid above $b(0)$ (since he gets the same status at a higher cost), no player wants to bid above the bid $b(0)$. That latter follows from the fact that the characterization in Lemma \ref{lem:myerson} guarantees that no player wants to deviate to any bid in the region of bids spanned by $b(\cdot)$ and hence $b(0)$. From this it immediately follows that they also don't want to bid above $b(0)$. Additionally, it is also trivial to see that no player wants to bid in the region $(0,\theta)$. Thus we can conclude that the above pair of interim allocation and contribution function are an equilibrium of the mechanism.

The fact that the badge mechanism has a unique equilibrium, follows from the recent results of Chawla and Hartline \cite{Hartline2012}. Despite the fact that general badge mechanisms do not fall into the class of auctions studied in \cite{Hartline2012} (such as for instance absolute threshold badge mechanisms), the specific leaderboard with a cutoff badge
mechanism fall into their framework. To show this, we need to argue that for any contribution profile $\bvec$ (even in the case of tied contributions), the ex-post expected allocation of status of a player depends only on his own contribution, on the number of players that have a higher contribution and on the number of players that have the same contribution (but for instance, not on the exact contributions of other players). Since, ties are broken uniformly at random, a player is ranked above another player with an equal contribution with probability of $1/2$. Thus if we denote with $n_g(\bvec)$ the number of players that contribute more and with $n_e(\bvec)$ the number of players with an equal contribution, then the expected ex-post status allocation of a player is:
\begin{equation*}
\sum_{\nu=0}^{n_e(\bvec)}\stat{\frac{n_g(\bvec)+n_e(\bvec)}{n-1}}\cdot \beta_{\nu,n_e(\bvec)}(1/2)
\end{equation*}
when his contribution $b_i\geq \theta$ and $0$ otherwise. It is clear that this ex-post allocation only depends on the quantities required by the framework of \cite{Hartline2012}.
\end{proof} 

Observe that the optimal badge mechanism described above has two main drawbacks. First the equilibrium contribution is a very complex function of the ability distribution, and therefore, small errors in a player's beliefs will dramatically change the total contribution that would arise in practice. Second, the optimal mechanism is not detail-free, as it depends on the monopoly quantile of the distribution. In the sections that follow we will address each of these issues separately and we will give approximately optimal badge mechanisms that avoid some of these drawbacks. 

Specifically, we will show that a very simple badge mechanism that is defined via an absolute contribution threshold, in a way that at equilibrium, half of the population acquires the top badge, is a $4$-approximation to the optimal badge mechanism when the status function is concave. For the players to decide how to play in this simple single absolute threshold mechanism it suffices to have correct beliefs only about the median ability, which seems a much smaller cognitive burden. We also address how a good approximation can be achieved by a multi-level absolute contribution threshold badge mechanism, with a small number of thresholds and even for convex status functions. Moreover, when the status function is convex, we show that the detail-free mechanism, that simply ranks the players in decreasing order of contribution (i.e. a leaderboard) achieves a $2$-approximation to the optimal total contribution.

%\begin{proof}
%\vsdelete{We note that the latter optimal mechanism can be implemented in the context of user-generated content as follows: simply rank players by contribution as long as they pass a threshold of contributions. All players that do not pass the threshold are assigned no status class. Since this is a symmetric ranking mechanism, the equilibrium will be unique and symmetric and monotone (see \cite{chawla2013auctions}). Thus players are essentially ranked by quantile, and hence the same allocation function as the optimal mechanism is implemented. Since the allocation is the same, the equilibrium bid of the players is equal to the one designated by the optimal mechanism by Equation \eqref{eqn:optimal-bid}. The contribution threshold is set to be equal to the bid of a player with quantile $\tqstar$, which by Equation \eqref{eqn:optimal-bid} is $\theta=\val(\tqstar)\cdot \statn{n}{\tqstar}$. }
%%Alternatively, the optimal mechanism can also be implemented by a continuum of badges with thresholds ranging from $\underline{\theta}=\val(\tqstar)\cdot \statn{n}{\tqstar}$ to $\overline{\theta}=\val(\tqstar)\cdot \xq{\tqstar}-\int_{0}^{\tqstar} \val(z)\xqpr{z}dz$.
%\end{proof}



%Equivalently, the optimal mechanism can be described in the quantile space, as ordering players in increasing quantile after
%discarding player with quantile higher than the quantile $\tqstar$ corresponding to the monopoly reserve $\eta$ and asking a player with quantile $\quant[i]$ to submit a bid of:
%\begin{equation}
%b_i(\quant[i]) = \val(\quant[i])\cdot \xq{\quant[i]}-\int_{1}^{\quant[i]} \xq{z}dz
%\end{equation}
%where\vsedit{
%\begin{equation}
%\xq{\quant[i]} = \sum_{\nu=0}^{n-1}\stat{\frac{\nu}{n-1}}\beta_{\nu,n-1}(\quant[i])
%\end{equation}}
%for any $\quant[i]\leq \tqstar$ and $0$ otherwise. 
%Last we also note that the revenue of the optimal mechanism can be computed through the use of the revenue function:
%\begin{equation}\label{eqn:optimal-revenue}
%\E_{\quant}\left[\sum_i b_i(\quant[i])\right]=n\int_{0}^{\tqstar} R'(\quant)\cdot \statn{n}{\quant}d\quant = n\left(R(\tqstar)\cdot \statn{n}{\tqstar}-\int_{0}^{\tqstar}R(\quant)\cdot\statnpr{n}{q}dq\right)
%\end{equation}





==> preliminaries-nsi.tex <==
% !TEX root=badges.tex

{\bf Optimal Mechanism Design.}  In the standard auction design problem, there are $n$ agents competing for a single unit of a divisible good.  The goal is to design an auction that maximizes {\em revenue} or total payments.  Each agent $i$ has a {\em value} $\val[i]$ per unit of the item drawn IID from an atomless distribution $\cdf$ with support $[0,\bar{\val}]$ and density $\pdf[\cdot]$.  Under this assumption, there is a one-to-one correspondence between an agent's value $\val[i]$ and his {\em quantile} $\quant[i]$:
$$
\quant(\val[i])=1-\cdf(\val[i]) \in [0,1]\mathrm{\ and\ }\val(\quant[i])=F^{-1}(1-\quant[i]).
$$ 
Intuitively, the quantile denotes the probability that a random sample from $\cdf$ has higher ability than agent $i$: thus lower quantile corresponds to higher value.  Note the distribution of quantiles is uniformly distributed in $[0,1]$.  As it is often more convenient to work in quantile space, we will henceforth state results using this terminology.

A direct revelation auction solicits {\em bids} $\bvec=(b_1,\ldots,b_n)$ from the agents and computes an allocation $\{x_i(\bvec)\}$ and set of payments $\{p_i(\bvec)\}$.  The resulting utility for agent $i$ with quantile $\quant[i]$ is then 
\begin{equation}
\label{eqn:standardutil}
u_i(\bvec;q_i)=\val(\quant[i])x_i(\bvec)-p_i(\bvec).
\end{equation}
Optimal auction design asks what allocation and payment rules maximize the total expected payments of the agents.  Answering this question requires a prediction of agent behavior: i.e., given a quantile and knowledge of the setting (distributions of other agents, auction rules, etc.), how will agents map quantiles to bids?  It is standard to predict that these maps, or {\em bidding strategies}, will comprise a {\em Bayes-Nash equilibrium} (BNE) of the underlying incomplete information game.  A profile of bidding strategies $b_i(\cdot)$ mapping quantiles to bids is a BNE if each agent maximizes their utility in expectation over the quantiles of the rest of the agents: for all $\quant[i]$, $b_i'$:
$$
\E_{\qvec_{-i}}\left[ u_i\left(\bvec(\qvec);\quant[i]\right)\right]\geq \E_{\qvec_{-i}}\left[u_i(b_i',\bvec_{-i}(\qvec_{-i});\quant[i])\right].
$$
This constraint gives rise to the standard characterization of BNE due to Myerson \cite{Myerson81} and Bulow and Roberts \cite{bulow1989simple}.  Letting $\hat{x}_i(\quant[i])=\E_\qvec[x_i(\bvec(\qvec));\quant[i]]$ and $\hat{p}_i(\quant[i])=\E_\qvec[p_i(\bvec(\qvec));\quant[i]]$ denote the {\em interim} allocation and payment rules respectively, the lemma  states:

\begin{lemma}[\cite{Myerson81}, \cite{bulow1989simple}]\label{lem:myerson-bne} A profile of contribution functions $\bvec(\cdot)$ and an implied profile of interim allocation and payment rules ${\bf \hat{x}}(\cdot)$ and ${\bf \hat{p}}(\cdot)$  are a BNE if and only if:
\begin{itemize}
\item $\hat{x}_i(\quant[i])$ is monotone non-increasing in $\quant[i]$ and
\item $\hat{p}_i(\quant[i]) = \val(\quant[i])\cdot \hat{x}_i(\quant[i]) + \int_{\quant[i]}^{1}\hat{x}_i(z)\cdot \val'(z)\cdot dz$
\end{itemize}
%The two conditions are also sufficient if the mapping $b(\cdot)$ spans the whole region of feasible contributions.
\end{lemma}

Simple manipulations of these identities allow one to characterize the revenue of a mechanism concisely in terms of the quantiles of the agents. Let $R(\quant)=\quant\cdot \val(\quant)$ denote the \emph{revenue function}\footnote{Intuitively, the revenue function computes the revenue a seller can generate by selling the (entire) item with probability $q$.} of the value distribution $\cdf[]$, and $R'(\quant[i])$ the \emph{virtual value} of a player.  Then,

\begin{lemma}[\cite{Myerson81}, \cite{bulow1989simple}]\label{lem:myerson-opt}
%The expected payment of each player is equal to his expected ``virtual allocation'': $\E_{\quant[i]}[b_i(\quant[i])]=\E_{\quant[i]}\left[R'(\quant[i])\cdot \hat{x}_i(\quant[i])\right]$, while 
The expected total payment of a mechanism is equal to the expected {\em virtual surplus}:
$$
\E_{\qvec}\left[\sum_i b_i(\quant[i])\right] = \E_{\qvec}\left[\sum_i R'(\quant[i])\cdot x_i(\qvec)\right].
$$
\end{lemma}

A consequence of Lemma~\ref{lem:myerson-bne}, known as {\em revenue equivalence}, is that if two mechanisms have the same interim allocation rule in BNE, they will also generate the same revenue.  A consequence of this observation and Lemma~\ref{lem:myerson-opt} is that the optimal mechanism is simply the mechanism maximizes the expected virtual surplus.  This reduces mechanism design to a constrained optimization problem.

For {\em regular} distributions $\cdf[]$, the form of the optimal mechanism is easy to describe.  A distribution $\cdf[]$ is \emph{regular} if the revenue function $R(\quant)=\quant \cdot \val(\quant)$, is a concave function, or equivalently, the virtual value of a player $R'(\quant)$ is non-increasing in his quantile.  Our assumption that $\cdf[]$ has support $[0,\bar{v}]$ also implies that $R(0)=R(1)=0$. Moreover, since virtual value $R'(\quant)$ is non-increasing in quantile, this implies that the virtual value is positive up until some quantile $\tqstar$, and negative afterwards. Quantile $\tqstar$, where $R'(\tqstar)=0$, is defined as the \emph{monopoly quantile} of the value distribution. Lemma~\ref{lem:myerson-opt} implies that the optimal mechanism only allocates to agents with quantiles below $\tqstar$.


==> preliminaries.tex.old.tex <==
% !TEX root=badges.tex

\paragraph{Ability Distribution and Quantile Space} We assume that each player's ability $\val[i]$ is private information and is drawn independently and identically from a commonly known, atom-less distribution $\cdf$ with support $[0,\bar{\val}]$ and density $\pdf[\cdot]$. Under this assumption, there is a one-to-one correspondence between a player's ability and his upper quantile:
\begin{equation}
\quant(\val[i])=1-\cdf(\val[i]) \in [0,1]
\end{equation}
Intuitively, the quantile denotes the probability that a random sample from $\cdf$ has higher ability than player $i$. Additionally, in the limit of a continuum of players, the quantile of a player denotes the proportion of players that have ability at least as high as him. Therefore, lower quantile corresponds to higher ability.

Due to the convenience of the quantile space in formulating mechanism design problems, we will work throughout the paper in the quantile space and we will instead, say that each player has a quantile $q_i$ drawn uniformly in $[0,1]$ and that his value is a function of his quantile, $\val(\quant[i])=F^{-1}(1-\quant[i])$, that depends on the distribution of abilities. Observe that $\val(0)=\bar{v}$ and $\val(1)=0$. A player's utility conditional on having quantile $\quant[i]$ is simply:
\begin{equation}
\hat{u}_i(\bvec;\quant[i]) = \stat{t_i(\rvec(\bvec))} - \frac{b_i}{\val(\quant[i])}
\end{equation}

\paragraph{Bayes-Nash Equilibrium and Translated Utility} Any badge mechanism defines a game of incomplete information among the $n$ players. We analyze the Bayes-Nash equilibria of this game. A BNE is a profile of mappings from
quantiles $\quant[i]$ to outputs $b_i(\quant[i])$ such that each player maximizes their utility in expectation over the quantiles of the rest of the players. For all $\quant[i]$, $b_i'$:
\begin{equation}
\E_{\qvec_{-i}}\left[ u_i\left(\bvec(\qvec);\quant[i]\right)\right]\geq \E_{\qvec_{-i}}\left[u_i(b_i',\bvec_{-i}(\qvec_{-i});\quant[i])\right]
\end{equation}
Since each player maximizes his utility conditional on his quantile, we can equivalently assume that a player's utility is:
\begin{equation}
u_i(\bvec;\quant[i]) = \val(\quant[i]) \cdot \hat{u}_i(\bvec;\quant[i]) = \val(\quant[i]) \cdot \stat{t_i(\rvec(\bvec))} - b_i
\end{equation}
because any strategy which maximizes their original utility $\hat{u}$ also maximizes $u$. This new formulation allows us to see that this game is equivalent to an all-pay auction where a player's allocation is a function of the status classes assigned to all players. 

Since the setting is symmetric from the perspective of every player, we focus on the symmetric Bayes-Nash equilibria of the game, where every player uses the same equilibrium mapping $b(\cdot)$. For a fixed symmetric equilibrium $b(\cdot)$, we denote with  $x_i(\qvec)=\stat{t_i\left(\rvec(\bvec(\qvec)))}\right)$, the ex-post status allocation of a player for a specific instantiation of player quantiles $\qvec$ and with $\hat{x}_i(\quant[i])=\E_{\quant[-i]}\left[x(q_i,\qvec_{-i})\right]$, the interim status allocation of player $i$, in expectation over the quantiles of the rest of the players. By symmetry of the equilibrium, the ability 
distribution and the auction rule, observe that the interim status allocation is the same function for all players and we denote it with $\xq{\quant[i]}$. Thus the expected utility of a player under a symmetric equilibrium is:
\begin{equation}
\E_{\qvec_{-i}}\left[u_i(\bvec;\quant[i])\right] = \val(\quant[i])\cdot \xq{\quant[i]}-b(\quant[i])
\end{equation}

\paragraph{Single-Parameter Optimal Mechanism Design} The latter formulation of the game defined by a badge mechanism, renders our setting a single-parameter mechanism design setting, with quasi-linear preferences $u_i(x_i,p_i) = v_i\cdot x_i - p_i$, where the allocation $x_i$ is the status allocation of a player and each player has a ''value'' $\val[i]$ per-unit of allocation equal to his ability and the payment of a player $p_i$ is his contribution. Moreover, under this relation, the total contribution objective is equivalent to the revenue of the mechanism. We now present a Lemma by Myerson \cite{Myerson81} and formulated in terms of quantiles by Bulow and Roberts \cite{bulow1989simple}, that characterize the equilibrium and the revenue of a mechanism will be very useful throughout our analysis. 
\begin{lemma}[\cite{Myerson81}, \cite{bulow1989simple}]\label{lem:myerson} A profile of contribution functions $\bvec(\cdot)=(b_1(\cdot),\ldots,b_n(\cdot))$ and an implied profile of interim allocation functions ${\bf \hat{x}}{\cdot}=(\hat{x}_1(\cdot),\ldots,\hat{x}_n(\cdot))$ are an equilibrium of a mechanism only if:
\begin{itemize}
\item $\hat{x}_i(\quant[i])$ is monotone non-increasing in $\quant[i]$ and
\item $b_i(\quant[i]) = \val(\quant[i])\cdot \hat{x}_i(\quant[i]) + \int_{\quant[i]}^{1}\hat{x}_i(z)\cdot \val'(z)\cdot dz$
\end{itemize}
The two conditions are also sufficient if the mapping $b(\cdot)$ spans the whole region of feasible contributions.

Moreover, if we denote with $R(\quant)=\quant\cdot \val(\quant)$, the \emph{revenue function} of the ability distribution $\cdf[]$, and with $R'(\quant[i])$ the \emph{virtual ability} of a player, then the expected contribution of each player is equal to his expected ``virtual allocation'': $\E_{\quant[i]}[b_i(\quant[i])]=\E_{\quant[i]}\left[R'(\quant[i])\cdot \hat{x}_i(\quant[i])\right]$, while the expected total contribution is equal to the expected ``virtual welfare'':
\begin{equation}
\E_{\qvec}\left[\sum_i b_i(\quant[i])\right] = \E_{\qvec}\left[\sum_i R'(\quant[i])\cdot x_i(\qvec)\right]
\end{equation}
\end{lemma}

\paragraph{Regularity, Revenue Function and Monopoly Quantile} Throughout the paper we will make the standard assumption in 
the auction design literature, that the distribution of abilities $\cdf[]$ is \emph{regular}, which concretely means that 
the revenue function $R(\quant)=\quant \cdot \val(\quant)$, is a concave function, or equivalently, that the \emph{virtual 
ability} of a player $R'(\quant)$ is non-increasing in his quantile. The regularity condition when expressed in the ability space states that the quantity: $\val-\frac{1-\cdf[\val]}{\pdf[\val]}$, is non-decreasing in $\val$. This is a weaker assumption than the Monotone Hazard Rate condition, assumed in Moldovanu et al. \cite{moldovanu2007contests}, which imposes that the hazard rate $\frac{\pdf[\val]}{1-\cdf[\val]}$ is non-decreasing in $\val$.

Our assumption that $\cdf[]$ has support $[0,\bar{v}]$ also implies that $R(0)=R(1)=0$. Moreover, since virtual ability $R'(\quant)$ is non-increasing in quantile, this implies that the virtual ability is positive up until some quantile $\tqstar$, and negative afterwards. Quantile $\tqstar$, where $R'(\tqstar)=0$, is defined as the \emph{monopoly quantile} of the ability distribution. Thus the revenue function is increasing in the region $\quant\in [0,\tqstar]$ and decreasing in the region $\quant\in [\tqstar,1]$.












==> robustness.tex <==
% !TEX root=badges.tex

\vscomment{This section is unfinished.}

So far we have assumed that the relation between input effort $e_i$ and quality of resulting submission $b_i$ is a deterministic one, $b_i=e_i\cdot v_i$. This implicitly assumes
that when a player decides to invest some amount of time on producing for instance a response to a Q\&A forum question, he knows ex-ante the exact quality of his submission.
Most of the times this is a hard assumption. Instead a player has a rough estimate on the resulting submission and there is some amount of noise.

We model such settings by saying that the relation between input effort and output submission is a stochastic one. Specifically, it is a linear relation up to a zero-mean noise, with some bounded
support. For ease of presentation assume that the relation is of the form:
\begin{equation}
b_i = v_i\cdot e_i + W_i
\end{equation}
where $W_i\sim U[-\epsilon,\epsilon]$, and we want to think of $\epsilon$ as a small constant. Our analysis will carry over to any distribution with support $[-\epsilon,\epsilon]$ and we
will denote such a noise distribution as $\epsilon$-bounded. Equivalently, we can think of the above game as the player choosing a target submission quality $b(v)=v\cdot e$ and then
nature adding some noise to this submitted quality, which yields the final bid of the player. 

In this section we claim that unlike the optimal mechanism, the badge mechanism is robust to noise in the following sense: there is a trivial additive translation of the noise-less
equilibrium strategy, that constitutes an $\epsilon$-equilibrium of the noisy game with an $\epsilon$-bounded noise. On the contrary we show that the latter doesn't hold for the optimal
mechanism.

\begin{theorem}Let $b(\cdot)$ be the symmetric equilibrium for a distribution of beliefs $F$ of the all-pay auction without any noise in the output. Then 
\begin{equation}
b^{\epsilon}(v) = b(v)+\epsilon
\end{equation}
is an $\epsilon$-equilibrium of the all-pay auction with an $\epsilon$-bounded noise, as long as $$2\epsilon<\min_{j} \{\theta_{j}-\theta_{j-1}\}.$$
\end{theorem}
\begin{proof}
Under $b^{\epsilon}(\cdot)$ the interim allocation of each player is exactly the same as under their interim allocation under $b(\cdot)$ in the game without any noise. The reason
being that the noise is never large enough to switch a player from a badge $j$ to a neighboring badge $j-1$ or $j+1$. Thus the number of players that congest badge $j$ is again
all players whose abilities are in the range $[a_j,a_{j+1})$, where value thresholds $a_j$ are the value thresholds corresponding to badge thresholds $\theta_j$ in the non noisy game.

If a player decreases his bid then his expected utility is at most 
\end{proof}

==> single.tex.old.tex <==
% !TEX root=badges.tex

In this section, we explore the approximate optimality of absolute threshold badge mechanisms that use a single badge. We prove that when status valuations are concave (including linear), a simple single badge mechanism with a particular threshold is a 4-approximation to the optimal mechanism. This threshold is set such that, in expectation, half of the population will earn the badge while the others will not. Furthermore, we show that a slightly more complex single absolute badge mechanism is a 2-approximation for linear status and a 3-approximation for strictly concave status. We also provide an example that shows this 2-approximation is tight for the case of linear status. 

Recall that an absolute threshold mechanism is characterized by a set of $k$ thresholds $\tbvec=(0,\tb{1},\ldots,\tb{k},\infty)$, such that $i$ is awarded badge $j$ if $b_i \in [\tb{j}, \tb{j+1})$. A single badge mechanism is characterized by a single threshold $\tb{}$ such that all users with $b_i >= \tb{}$ earn the badge. We begin our analysis by characterizing the Bayes-Nash equilibria of an absolute threshold mechanism with thresholds $\theta_1,\ldots,\theta_m$. We focus on symmetric equilibria\footnote{We note that asymmetric equilibria do exist in our setting, even in the case of a single badge and two players distributed $U[0,1]$.} and show there is a unique symmetric equilibrium. This equilibrium is monotone, non-increasing in each player's quantile. Recall that a lower quantile implies a higher ability, so the higher ability players will contribute more than lower ability players in this equilibrium. 
%
% which is monotone, i.e. each player uses the same strategy mapping $b_i(\quant[i]) = b(\quant[i])$ and this mapping is monotone non-increasing in the player's quantile. More generally, the purpose of this section is to show the following theorem.

\begin{theorem}\label{thm:uniqueness}
Every vector of contribution thresholds $\tbvec=(\tb{1},\ldots,\tb{m})$ has a unique symmetric BNE characterized by quantile thresholds $\tqvec=(\tq{1},\ldots,\tq{p})$ for some $p\leq m$, such that $b(\quant[i])=\theta_t$ if $\quant[i]\in (\tq{t+1},\tq{t}]$. Moreover, for any vector of quantile thresholds $\tqvec=(\tq{1},\ldots, \tq{p})$ there exists a set of contribution thresholds under which the unique symmetric BNE is characterized by $\tqvec$.
\end{theorem}


Observe that in this mechanism there are only two contribution levels in equilibrium, which are $\theta$, the threshold for earning the badge, and 0. Increasing a user's contribution above $\theta$ yields no additional gain in status and only costs the agent effort.. 

For any contribution threshold $\theta$, there exists a corresponding quantile threshold $\tq{}$ such that 

We first argue that such a mechanism has a unique symmetric equilibrium.\footnote{We note that asymmetric equilibria do exist in our setting, even in the case of a single badge and two players distributed $U[0,1]$.} Observe that by Lemma \ref{lem:myerson}, both the expected status allocation and the equilibrium contribution function has to be non-increasing in
quantile. In the single absolute threshold mechanism, the only contributions that make sense for a player to submit are either
$0$ or $\theta$, since by submitting any other contribution in between, he gets the exact same status allocation and at a strictly higher cost. Thus the equilibrium bid function must take the form: $b(\quant)=\theta\cdot {\bf 1}_{\quant\leq \tq{}}$, for some 
quantile threshold $\tq{}$. Under such an equilibrium, the interim allocation of status of a player will simply be: $\xq{\quant}=\statn{n}{\tq{}}\cdot {\bf 1}_{\quant\leq \tq{}}$, since the proportion of players that get at least as high 
badge as a player $i$ with quantile $\quant\geq \tq{}$ is exactly the proportion of players that have quantile above $\tq{}$. By Lemma \ref{lem:myerson}, for such a contribution and interim allocation function to be at equilibrium it must hold that:
\begin{equation}\label{eqn:contribution-quantile-single}
\theta = \val(\tq{})\cdot \statn{n}{\tq{}}
\end{equation}
Observe that the right hand side is a strictly decreasing function of $\tq{}$. Therefore, the above equation has a unique solution  
if $\theta<\bar{v}\cdot \stat{0}$ and no solution otherwise (in which case no-one submits a contribution of $\theta$).

\begin{corollary}

For any contribution thresholds $\theta$, there exists quantile thresholds $\tq{}$ such that in the unique symmetric equilibrium, all players with quantile $\quant \leq \tq{}$ contribute $\theta$ and earn the badge while all other players contribute 0. For any quantile threshold $\tq{}$, there is a contribution threshold 
%For any contribution threshold $\theta$ the single absolute contribution threshold badge mechanism has a unique symmetric equilibrium characterized by a quantile threshold $\tq{}$, such that all players with quantile $\quant\leq \tq{}$, submit contribution $\theta$ and all remaining players make no contribution. The converse is also true.
\end{corollary}
In the next section, we generalize the above uniqueness result to a multi-level absolute contribution threshold mechanism. In the remainder of the section we will refer to an absolute contribution mechanism by it's quantile threshold, rather than it's contribution threshold. By applying Equation \eqref{eqn:contribution-quantile-single} we get the contribution threshold that the designer needs to set to implement the corresponding quantile threshold. 

\paragraph{An Illustrative Case: Linear Status}\label{sec:linear}
To illustrate the main technical insights of the main result of this section, we start by analyzing the very illustrative case of linear status. 
\begin{equation}
\stat{t} = 1-t.
\end{equation}
That is, a player's status value is simply the proportion of players that she beats. Apart from its simplicity, linear status has a natural interpretation as argumentative power in Q\&A forums: it corresponds to the probability that a player wins an argument against a random other participant of the forum and assuming that in such an argument the player with the higher badge wins and if both players have the same badge then they both lose (a more elaborate analysis of this connection, and variants of it, is given in Section \ref{sec:tie-breaking}). 

In the linear status case the interim allocation of the optimal mechanism takes the simple form: $\xq{\quant}=\statn{n}{\quant}\cdot {\bf 1}_{\quant\leq \tqstar}=(1-\quant)\cdot {\bf 1}_{\quant\leq \tqstar}$ and therefore the optimal per
player contribution is:
\begin{equation}\label{eqn:linear-optimal-revenue}
\opt =  \int_0^{\tqstar} R'(\quant)\cdot \statn{n}{\quant}d\quant = R(\tqstar)\cdot (1-\tqstar) +\int_{0}^{\tqstar}R(\quant)d\quant
\end{equation}
On the other hand the per player contribution of a single absolute threshold threshold mechanism with quantile threshold
$\tq{}$, is:
\begin{equation}
\apx = \tq{}\cdot \theta = R(\tq{})\cdot \statn{n}{\tq{}}=R(\tq{})\cdot (1-\tq{})
\end{equation}
Thus, showing that a single absolute badge can well approximate the optimal mechanism, boils down to showing the existence
of a quantile threshold $\tq{}$, such that the above two portions are always within a constant factor.

Observe that by setting $\tq{}=1/2$, then $\apx=\frac{1}{2}R(1/2)$. By concavity of the revenue function and applying Jensen's inequality, we get that $R(1/2)\geq \int_0^{1}R(\quant)d\quant$. Additionally, since $R(0)=R(1)=0$, it is easy to see that $\int_0^1 R(\quant)d\quant \geq \frac{1}{2}\cdot R(\tqstar)$.\footnote{This is the same argument
employed for proving the statement that the revenue of the optimal single item auction with a single bidder yields lower revenue than the second price auction with two i.i.d bidders. See Figure 5.1 in \cite{Hartline2012}} On the other hand, by Equation \eqref{eqn:linear-optimal-revenue}, and since $\statn{n}{\quant}\leq 1$, it is easy to see that $\opt\leq R(\tqstar)$. This leads to the following corollary.

\begin{corollary}[Median Absolute Badge Mechanism]\label{cor:median-linear}
When the status function is linear, a single absolute badge mechanism with quantile threshold $\tq{}=1/2$ achieves a $4$-approximation to the optimal revenue.
\end{corollary}
In the next section we generalize the latter result to any concave status function. As the following example shows, the latter $4$-approximation is tight, when the ability distribution is very dispersed and high ability players are very rare.

\begin{example}[Tight lower bound for median badge mechanism] Consider the case of a linear status function $\stat{t}=1-t$ and a distribution of abilities with density function $F(\val)=\frac{H+1}{H}\frac{\val}{\val+1}$ and support
$[0,H]$. The value function of this distribution is $\val(\quant)=\frac{1-\quant}{\frac{1}{H}+\quant}$ and the revenue function is $R(\quant)=\frac{\quant}{\frac{1}{H}+\quant}\cdot (1-\quant)$. As $H\rightarrow \infty$ (abilities are very dispersed but most of the mass is at the lower end) the revenue curve converges to $R(\quant)\rightarrow (1-\quant)$ and the optimal per player contribution converges to $1$. On the other hand the per player contribution of the median badge converges to $\frac{1}{4}$.
\end{example}
\begin{figure}[htpb]
\centering
\subfigure{\includegraphics[scale=.75]{4-lower-bound-opt.eps}}
\subfigure{\includegraphics[scale=.75]{4-lower-bound-apx.eps}}
\caption{Left figure depicts the per player contribution of the optimal badge mechanism, when the cdf of the ability distribution is of the form $\cdf[\val]=\frac{H+1}{H}\frac{v}{v+1}$. The monopoly quantile is $\tqstar=\frac{\sqrt{1+H}-1}{H}\rightarrow 0$ as $H\rightarrow 0$, while $R(\tqstar)\rightarrow 1$. The per player contribution of a single absolute badge at $\kappa=1/2$ is depicted on the right and as  $H\rightarrow 0$, it is a quarter of the optimal per player contribution.} \label{fig:linear}
\end{figure}

The latter lower bound shows that in order to get a better approximation to the optimal contribution, we also need to take into account the form of the revenue function and more specifically, whether the monopoly quantile is below $1/2$. This leads to the following improved single absolute badge mechanism.

\begin{theorem}\label{lem:linear}
When the status function is linear, a single absolute badge with quantile threshold $\tq{}=\min\{\tqstar,1/2\}$ achieves a $2$-approximation to the optimal revenue. (proof in Appendix)
\end{theorem}

A graphical depiction of the latter $2$-approximation theorem is given in Figure \ref{fig:linear}. 
%The latter theorem can also be easily generalized to show that if $m$ badges are used, then a $\frac{m+2}{m}$ approximation is achieved.
%, by placing badges at quantile thresholds: $\tq{t}=\min\{\tqstar,\frac{t}{m+1}\}$, $t\in[1,m]$ for any even $m$.
\begin{figure}[htpb]
\centering
\subfigure{\includegraphics[scale=.75]{half-approx-graphic.eps}}
\subfigure{\includegraphics[scale=.75]{half-approx-apx.eps}}
\caption{Left figure depicts the per player contribution of the optimal badge mechanism, when the ability distribution is of the form $\cdf[\val]=\val^{\alpha}$. Observe that the rectangle
with height $R(1/2)$ is at least as large as the area below the concave curve, since the curve lies below the
tangent at $1/2$. The per player contribution of a single absolute badge at $\kappa=1/2$ is depicted on the right and is half of the latter rectangle. As $\alpha\rightarrow \infty$, the left area converges to a triangle, and no single badge can achieve more than a half approximation.} \label{fig:linear}
\end{figure}

\begin{example}[Tight lower bound for any single absolute threshold] We give a distribution of abilities, where the bound of $2$ proved in Theorem \ref{lem:linear} is tight. In fact the 
example shows that no single badge mechanism can yield better than a $2$-approximation. Consider a distribution of abilities with density function 
$F(v)=v^{\alpha}$, ($\alpha\in [1,\infty]$) and support $[0,1]$. The ability as a function of the quantile is then $\val(\quant)=(1-\quant)^{1/\alpha}$
and the revenue function is $R(\quant)=\quant \cdot (1-\quant)^{1/\alpha}$. As $\alpha\rightarrow \infty$ (i.e. as the distribution converges to a point
mass at $1$), then we get that $R(\quant)\approx q$. 
Hence, the per player contribution of the optimal mechanism will converge to $\int_0^1 \quant\cdot d\quant = \frac{1}{2}$. On the other hand, the per player contribution of any single absolute badge mechanism is $R(\tq{})=\tq{} \cdot (1-\tq{})\leq \frac{1}{4}$. This lower bound also has an intuitive graphical representation
as in Figure \ref{fig:linear}, where pictorially, the revenue curve will converge to the identity function.
\end{example}

\paragraph{Concave Status} The results presented in the previous section extend qualitatively to the case of any general concave status function. Concavity of the status function implies that the marginal increase from beating one extra person decreases as a player is closer to the top. Hence, it is intuitive that for such status functions
a very coarse status discrimination is sufficient to incentivize players to invest close to the optimal effort. We start by extending Corollary \ref{cor:median-linear} and then show that Theorem \ref{lem:linear} also extends with small degradation in the approximation factor.

\begin{theorem}\label{thm:concave} If the social status function is concave, then a single badge, with quantile threshold of $1/2$, achieves a $4$-approximation to the optimal total contribution. 
\end{theorem}
\begin{proof}
By the analysis similar to the linear case, we remind that the per-player contribution of single badge mechanism is:
$\apx=R(1/2)\cdot \statn{n}{1/2}$, while the optimal per player contribution is upper bounded by $\opt\leq R(\tqstar)\cdot \statn{n}{0}$.

As we showed in the linear case, by concavity of the revenue function and by the fact that $R(0)=R(1)=0$: $R(1/2)\geq \frac{1}{2}R(\tqstar)$. Moreover, the fact that $\stat{\cdot}$ is a decreasing concave function with $\stat{1}=0$, implies as 
already noted in the previous section that, $\statn{n}{\cdot}$ is also decreasing concave with
$\statn{n}{1}=0$. Thus, $\statn{n}{1/2}\geq \frac{1}{2}\statn{n}{0}$. The theorem then follows.
\end{proof}

A substantially more involved analysis, which we defer to the Appendix, shows that if we also take into account the 
monopoly quantile of the distribution, then a better $3$-approximation guarantee can be achieved.
\begin{theorem}\label{thm:concave} If the social status function is concave, then a single badge, with quantile threshold of $\min\{\tqstar,1/2\}$, achieves a $3$-approximation to the optimal total contribution. (proof in Appendix)
\end{theorem}
